A Unified Fading Model Using Infinitely Divisible Distributions

This paper proposes to unify fading distributions by modeling the magnitude-squared of the instantaneous channel gain as an infinitely divisible random variable. A random variable is said to be infinitely divisible, if it can be written as a sum of $n \geq 1$ independent and identically distributed random variables, for each $n$. Infinitely divisible random variables have many interesting mathematical properties, which can be applied in the performance analysis of wireless systems. It is shown that the proposed unification subsumes several unifications of fading distributions previously proposed in the wireless communications literature. In fact, almost every distribution used to model multipath, shadowing and composite multipath/shadowing is shown to be included in the class of infinitely divisible random variables.

==> abstract.tex <==
Stochastic orders are binary relations defined on probability
distributions which capture intuitive notions like being larger or
being more variable. This paper introduces stochastic ordering of
instantaneous SNRs of fading channels as a tool to compare the
performance of communication systems over different channels.
Stochastic orders unify existing performance metrics such as ergodic
capacity, and metrics based on error rate functions for commonly
used modulation schemes through their relation with convex and
completely monotonic (c.m.) functions. Toward this goal, performance
metrics such as instantaneous error rates of $M$-QAM and $M$-PSK
modulations are shown to be c.m. functions of the instantaneous SNR,
while metrics such as the instantaneous capacity are seen to have a
completely monotonic derivative (c.m.d.). It is shown that the
frequently used parametric fading distributions for modeling line of
sight (LoS) exhibit a monotonicity in the LoS parameter with
respect to the stochastic Laplace transform order. Using stochastic
orders, average performance of systems involving multiple random
variables are compared over different channels, even when closed
form expressions for such averages are not tractable. These include
diversity combining schemes, relay networks, and signal detection
over fading channels with non-Gaussian additive noise, which are
investigated herein. Simulations are also provided to corroborate
our results.


==> paper_body_bak.tex <==
\section{Introduction}
\label{sec:Intro}
Practical wireless communications systems are typically subject to multiple channel impairments, of which multipath fading is one of the most important. In analyzing the performance of such systems, empirical stochastic models such as Rayleigh, Rician and Nakagami-$m$ distributions have been proposed to capture the distribution of the envelope of the fading random variable (RV). Since these distributions have been proposed through empirical means, it is unknown as to whether all the fading distributions belong to a common subclass of probability distributions. Through a unification of fading distributions, it may be possible to obtain canonical expressions for the performance metrics of fading channels, thereby simplifying the analysis of fading channel systems. In addition, it is possible that such a unification may provide insight into the physical basis behind the empirical fading distributions. Last, but not the least, the unified model may permit us to compare two different fading distributions with respect to system performance metrics such as the average symbol error rate (SER), using the technique of stochastic ordering. Stochastic orders are partial orders on RVs, which are based on comparisons of the expectations of functions of RVs, and their applications to fading channel ordering have been discussed in \cite{paper:adithyaSTpaper}. Therefore, it seems compelling to develop a unified study of fading distributions with these goals in mind.

There have been multiple efforts toward unifying fading distributions in the past. Typically, the magnitude of the fading RV (which we call as the envelope), or the magnitude-square of the fading RV (referred to as instantaneous {\effch}) has been modelled as a mixture of more than one distribution. To be more specific, one of the unified models - the spherically invariant random process has been proposed as a general model which attempts to capture a fading envelope RV as variance mixture of a Rayleigh RV \cite{yao2004unified}; a unification proposed in \cite{paper:alouini} models the instantaneous {\effch} RV as the product of a gamma RV and a generalized-gamma RV. While this model encompasses many known fading distributions, it does not include some distributions such as the Pareto distribution, which has been used in \cite{pun07}. Another unification in the literature is the generalized gamma distribution (also known as the Stacy distribution \cite{stacy1962generalization}), which is shown to correspond to the distribution of the envelope, when the received signal is composed of clusters of multipath components, wherein the receiver possesses power-law nonlinearity \cite{yacoub2007alpha}. While this is a physically motivated fading model, it does not include fading distributions such as the Pareto distribution and the Beta distribution, which are known to occur in certain wireless interference scenarios \cite{pun07, ghasemi2006capacity}. There are several other references where a unified fading model is proposed \cite{paper:Nstarnakagami, sagias2006performance}. However, they do not include some popularly used fading distributions such as the Rician distribution.

For the first time in the literature, we propose to unify fading distributions by modeling their instantaneous {\effch} as an infinitely divisible (ID) RV. A RV is said to be infinitely divisible, if it can be written as a sum of $n \geq 1$ independent and identically distributed (i.i.d.) RVs, for each $n$. Intuitively, this means that the channel can be viewed as a (time/frequency/antenna) diversity combining system with $n$ i.i.d. channels, for every $n \geq 1$. Infinitely divisible RVs have many interesting mathematical properties, and have been extensively studied in the statistics literature (See \cite{book:steutel2003infinite} and the references therein). We, for the first time in the literature, observe that, within the class of ID RVs, a very special subclass, known as generalized gamma convolutions (GGCs) includes almost every fading distribution. Consequently, we pay special attention to this subclass of ID RVs. Formally, GGCs are defined as the weak limits of finite convolutions of Gamma distributions, and have been thoroughly studied in \cite{book:bondessonGGC, bondesson1988remarkable, bondesson1990generalized, james2008generalized}. There are numerous applications of GGCs in financial economics \cite{barndorff2001non, carr2001optimal, figueroa2004nonparametric} and risk analysis \cite{burmaster1996introduction, schroder2004risk}. Even though GGCs possess remarkable structure and properties which are relevant to fading channel analysis, no applications of this set of distributions has been found in the wireless communications literature. 

The class of GGCs includes a surprisingly large number of fading models such as the lognormal, Rayleigh, Nakagami-$m$, generalized gamma distribution, Pareto, Beta, inverse Gaussian and the positive $\alpha$-stable distributions. Moreover, multiplicative mixture fading models such as Rayleigh-lognormal, Nakagami-lognormal, and special cases of the spherically invariant random process, and the generalized model proposed in \cite{paper:alouini} are also GGCs. From a wireless perspective, if a system has GGC distributed instantaneous {\effch}, then the fading channel is equivalent to a coherent linear combination of (possibly infinitely) many independent branches where the instantaneous fading power is gamma distributed. Another physical interpretation we will show, is the following: if a channel with finite multipath diversity order has a GGC distributed instantaneous {\effch}, then the channel is equivalent to a Nakagami-$m$ fading model, where $m$ is a RV. Unifying instantaneous {\effch} distributions as GGCs, it is possible for us to obtain novel generalized expressions for performance metrics of wireless systems, such as the ergodic capacity and the average SER. Furthermore, this unification reveals new stochastic ordering relations applicable to members of GGC. Lastly, we obtain conditions under which systems composed of multiple fading RVs, such as diversity combining schemes have GGC end-to-end instantaneous {\effch}. This facilitates us to obtain bounds on the performance of such systems.

The rest of the paper is organized as follows. In Section \ref{sec:MathPreliminaries}, the required mathematical background, including a short exposition of generalized gamma convolutions is presented. Section \ref{sec:GGCandHCMChannels} provides the detailed justification and intuition behind using GGCs as a unified model for fading. In addition, several examples of fading distributions used in the literature are shown to be GGCs in this section. We then provide some analytical expressions for performance metrics of GGC fading channels in Section \ref{sec:GGC_performanceMetrics}. Section \ref{sec:OrderingGGCs} describes some new stochastic ordering relations applying to GGC RVs. In Section \ref{sec:GGCPerfBoundsSys}, we consider multi-antenna systems such as maximum ratio combining (MRC), equal gain combining (EGC) and selection combining (SC). Finally, we provide Monte-Carlo simulations to corroborate some of our results in Section \ref{sec:simulations} and summarize our conclusions in Section \ref{sec:conclusions}. 

\subsection{Notations and Conventions}
\label{sec:notations}
The set of real numbers and positive integers are denoted by $\re$ and $\N$ respectively, while all other sets are denoted using script font. For a Radon measure $\mu(\cdot)$, $\mu(u)$ is used to represent $\mu([0,u])$. For a RV $X$, the cumulative distribution function (CDF) and the probability density function (PDF) are denoted by $\CDF{X}{\cdot}$ and $\pdf{X}{\cdot}$ respectively. $\E{}{g(X)}$ is used to denote the expectation of the function $g(\cdot)$ over the PDF of $X$. The Laplace transform and Laplace exponent of a nonnegative RV $X$ are defined as $\MGF{X}{\cdot} = \E{}{\exp(-s X)}$ and $\gamma_{X}(s) = -\log \E{}{\exp(-s X)}$ respectively, which are defined for $s \geq 0$. All logarithms are natural logarithms. We write $f_{1}(x) = O(f_{2}(x))$, $x \rightarrow a$ to indicate that $\limsup_{x \rightarrow a} (f_{1}(x)/f_{2}(x)) < \infty$, and $f_{1}(x) \sim f_{2}(x)$, as $x \rightarrow a$ to indicate $\lim_{x \rightarrow a}f_{1}(x)/f_{2}(x) =1$. Throughout, we adopt the convention that $0 \cdot \infty = 0$.
\section{Mathematical Preliminaries}
\label{sec:MathPreliminaries}
\subsection{Bernstein Functions}
A function $g: \re^{+} \rightarrow \re^{+}$ is said to be completely monotone (c.m.) if it has derivatives of all orders, which satisfy $(-1)^{k}\D^{k} g(x)/ \D x^{k} \geq 0$, for $k=0,1,2,\ldots$. According to Bernstein's theorem, every c.m. function is characterized as a mixture of decaying exponential functions \cite{book:schilling}. Many performance metrics of communication systems such as SERs of $M$-QAM and $M$-PSK are {\cm} functions of the average SNR \cite{paper:adithyaSER}.

If a function $g: \re^{+}\rightarrow \re^{+}$  is such that $\D g(x) / \D x$ is c.m., then it is known as a Bernstein function \cite{book:schilling}. Every Bernstein function can be written in the form
\begin{align}
\label{eqn:bern_characterize}
g(x) = a + bx  + \int\limits_{0}^{\infty} (1-\exp(-ux))\tau(\D u)\;,
\end{align}
for some $a,b \geq 0$, and a non-negative measure $\tau$ on $(0,\infty)$ which satisfies $\int_{0}^{1}\tau(\D u) + \int_{1}^{\infty} u \tau( \D u) < \infty$. In this case, $\tau$ is known as the Levy measure of $g$. Bernstein functions are relevant to this work, because the Laplace exponents of non-negative infinitely divisible RVs introduced in Section \ref{sec:GGC_intro}, are Bernstein functions.

The subset of Bernstein functions, for which $u \tau(u)$ is c.m., constitutes the set of Thorin-Bernstein functions $\TBF$. Any function in this set admits the following representation, in addition to \eqref{eqn:bern_characterize}:
\begin{align}
\label{eqn:TBF_characterize}
g(x) = a + bx  + \int\limits_{0}^{\infty} \log(1+s x) \mu (\D s)\;,
\end{align}
for some non-negative $a,b$, and a non-negative measure $\mu$ on $(0,\infty)$ which satisfies $\int_{0}^{1}|\log s | \mu(\D s) + \int_{1}^{\infty}s \mu(\D s)< \infty$. In this case, $\mu$ is called the Thorin measure of $g$. In this work, we refer to $\int_{0}^{\infty} \mu(\D s)$ as the \emph{mass} of the Thorin measure, or the \emph{Thorin mass}.

An example of a Thorin-Bernstein function relevant to wireless communications is $g(x) = \log(1+x)$. This is because, if we view $\rho X$ as the instantaneous SNR of a channel, where $\rho$ is the average SNR, then $\E{}{g(\rho X)}$ represents the ergodic capacity of the channel.
\subsection{Regular Variation}
We very briefly touch upon some concepts from regular variation theory, which we will be making use of, in Section \ref{subsec:GGCGenGammaIntro}.

A real valued function $H(x) : \re^{+} \mapsto \re^{+}$ is said to be regularly varying at $\infty$ (or at $0$) if $\lim_{x \rightarrow \infty} H(tx)/H(x)$ (or $\lim_{x \rightarrow 0} H(tx)/H(x)$) exists, and is equal to $t^{r}$, with $0 < |r| < \infty$. It is said to be slowly varying at $\infty$ (or at $0$) if $r=0$. If $H$ is differentiable with $h(x) = \D H(x)/\D x$, and $h(x) = m x^{m-1} l(x)$, where $l$ is slowly varying at $0$, then $H(x) \sim x^{m} l(x)$, as $x \rightarrow 0$. 
\subsection{Infinite Divisibility and Generalized Gamma Convolutions}
\label{sec:GGC_intro}
\subsubsection{Infinite Divisibility}
A probability distribution is said to be infinitely divisible (ID) if, for each $n \geq 1$, it can be decomposed into $n$ identical convolution factors. Some examples of such distributions are the Gamma, the Poisson and the Gaussian distributions. In this paper, we refer to RVs with ID distributions as ID RVs. Non-negative ID RVs are characterized by the fact that the Laplace exponents of such RVs are Bernstein functions. Non-negative ID RVs are very relevant from a wireless communications context, because it is intuitive to expect a fading channel to possess an ID instantaneous {\effch}. This is because it is conceivable to view fading as the resulting effect of coherent combination of contributions from multiple different sources. Coincidentally, almost all known instantaneous {\effch} distributions are ID, some examples of which are listed below.
\begin{example}
The instantaneous {\effch}s corresponding to Rician-$K$, Nakagami-$m$ and lognormal fading are ID.
\end{example}
\begin{proof}
The Infinite divisibility of the lognormal RV has been shown in \cite{thorin1977infinite}. For the case of Nakagami-$m$ fading, the instantaneous {\effch} is a Gamma RV with LT $\MGF{}{s} = \exp(-m \log(1+s/m))$. It is easy to show that the Laplace exponent $\gamma_{\mathrm{N}}(\rho) = m \log(1+s/m)$ can be written in the form \eqref{eqn:bern_characterize} with $a=b=0$ and $\tau(\D u) = m \exp(-m t)\D t/t$ \cite[p. 228]{book:schilling}. Therefore, the Laplace exponent is a Bernstein function, and consequently, the instantaneous {\effch} corresponding to Nakagami-$m$ fading is an ID RV.

Next, we address the case of Rician-$K$ fading. The LT of the instantaneous {\effch} for this case is given by \cite[p. 19]{simon_alouini05}
\begin{align}
\MGF{}{\rho} = \frac{1+K}{1+K+\rho} \exp\left( - \frac{K \rho}{1+K+\rho}\right)\;,
\end{align}
from which the Laplace exponent is obtained as
\begin{align}
\gamma_{\mathrm{R}}(\rho) = \frac{K \rho}{1+K+\rho}+ \log\left(1+ \frac{\rho}{1+K} \right)\;.
\end{align}
Using Frullani's representation for $\log(1+x)$ \cite[p. 6]{book:lebedev72}, it is straightforward to show that $\gamma_{\mathrm{R}}(\rho)$ can be written in the form \eqref{eqn:bern_characterize} with $a=b=0$ and 
\begin{align}
\tau(\D u) = \exp(-(1+K)u)\left( K(1+K)+\frac{1}{u}\right) \D u\;.
\end{align}
Therefore, $\gamma_{\mathrm{R}}(\rho)$ is a Bernstein function, and consequently, the instantaneous {\effch} corresponding to Rician-$K$ fading is an ID RV.
\end{proof}
To the best of our knowledge, the proof of infinite divisibility of the instantaneous {\effch} for the Rician-$K$ case has not been found elsewhere in the literature. On the other hand, the infinite divisibility of the instantaneous {\effch} for Nakagami-$m$ fading is straightforward to see, and that for the lognormal case is known in the literature. Nevertheless, we provide it here for the sake of completeness. In fact, the infinite divisibility of the lognormal distribution, proved by Thorin \cite{thorin1977infinite} revealed a very rich class of ID probability distributions known as generalized gamma convolutions (GGC), which possess extremely useful mathematical properties applicable to wireless systems. In addition, several popularly used fading distributions are not only ID, but also GGC. This fact motivates us to consider this very special class of ID distributions, which is discussed next. 
\subsubsection{Generalized Gamma Convolutions}
\label{subsec:GGCGenGammaIntro}
The subset of non-negative ID distributions for which the Laplace exponent belongs to $\TBF$, constitutes the set $\GGC$ of GGC probability distributions. In other words, the LT of the RV admits the form 
\begin{align}
\label{eqn:MGF_GGC_gen}
\phi(s) = \exp \left(-as-\int\limits_{0}^{\infty}\log(1+s/u) \mu(\D u) \right)\;,
\end{align} 
where the parameters $a \geq 0$, and $\mu(\cdot)$ (nonnegative measure on $[0,\infty)$) uniquely characterize the GGC distribution. In this paper, we call the Thorin measure of the Laplace exponent of the GGC (e.g. $\mu$ in \eqref{eqn:MGF_GGC_gen}) as the Thorin measure of the GGC. 

In a wireless context, the Thorin measure of a GGC has a physical interpretation: Consider the case where a continuum of fading channels with Gamma distributed instantaneous power is coherently summed up. If the sequence of shape parameters corresponding to each rate parameter $u$ in $[0,\infty)$ of the Gamma distributed channels is $\mu(u)$, then the Thorin measure of the GGC channel is $\mu$. From a mathematical perspective, the Thorin measure determines performance metrics such as the average symbol error rate and ergodic capacity, as we will show in Section \ref{sec:GGC_performanceMetrics}. Furthermore, a close interplay between the stochastic ordering of GGCs and their Thorin measures is observed, as discussed in Section \ref{sec:OrderingGGCs}.

In what follows, we will restrict our attention to GGCs with $a=0$, because $a$ merely represents a translation of the instantaneous {\effch} PDF, and performance analysis for such channels can be obtained from systems where $a=0$ using straightforward algebra. 

From the perspective of this work, the variation exponent of the LT of the GGC near infinity is useful, and this quantity relates to the Thorin measure as follows:
\begin{lem}{{\cite[Theorem 4.1.4]{book:bondessonGGC}}}
\label{lem:GGC_thorinmass}
The LT of a non-degenerate GGC is regularly varying near $\infty$, and the variation exponent equals the Thorin mass. That is, $\lim_{\rho \rightarrow \infty} \MGF{}{t \rho}/\MGF{}{\rho} = t^{-c_{0}}$, where
\begin{align}
c_{0} = \int\limits_{0}^{\infty}\mu (\D s) 
\end{align}
%Equivalently, the variation exponent of $\pdf{X}{x}$ near the origin is $\alpha-1$, where $\alpha$ is the Thorin mass of the GGC.
\end{lem}
In the context of a wireless system, the variation exponent of the average error rate near infinity has been proposed as a generalized definition of diversity order. Since the LT of the instantaneous {\effch} equals twice the average SER of DPSK, from Lemma \ref{lem:GGC_thorinmass}, we see that the diversity order of DPSK over a GGC fading channel is equal to its Thorin mass. 

The Thorin measure also determines the expected value of a GGC RV:
\begin{proposition}
\label{thm:AvgPwr}
Let X be a non-degenerate GGC. Then $\E{}{X} = \int_{0}^{\infty}  \mu(\D u)/u $, if the integral is finite.
\end{proposition}
\begin{IEEEproof}
%Differentiating the LT of a GGC and evaluating the derivative near the origin, we see that
%\begin{align}
%\int\limits_{0}^{\infty} x \pdf{X}{x} \D x = \lim_{s \rightarrow 0} \exp ( \int \log (1+s/u) \mu(u) \D u) \left(\int\limits_{0}^{\infty}  \mu(u) /u(1 + s u) \D u \right), 
%\end{align}
%which equals $\int_{0}^{\infty}  \mu (u)/u \D u$, if the integral is finite.
It is easy to show for any nonnegative RV that $\E{}{X} = -\lim_{\rho\rightarrow 0} \D \MGF{X}{\rho}/\D \rho$. Since the LT of a GGC is of the form $\MGF{X}{\rho} = \exp(-\gamma(\rho))$, we get $\E{}{X} = \lim_{\rho \rightarrow 0} \D \gamma(\rho)/\D \rho$, where $\gamma(\cdot)$ is the Laplace exponent of the GGC. Representing $\gamma$ in terms of the Thorin measure, we get
\begin{align}
\E{}{X}  = \lim_{\rho \rightarrow 0} \int\limits_{0}^{\infty} \frac{1/u}{1+\rho/u} \mu(\D u)\;,
\end{align}
where $\mu$ is the Thorin measure. The limit and integral can be interchanged if 
\begin{align}
\label{eqn:GGCMeanDC}
\int_{0}^{\infty} u^{-1} \mu(\D u) < \infty \;,
\end{align}
because under this condition dominated convergence is satisfied. Assuming \eqref{eqn:GGCMeanDC} to be true, we interchange the limit and integration to yield the Proposition.
\end{IEEEproof} 
If $X$ represents the instantaneous {\effch} in a fading system, then Proposition \ref{thm:AvgPwr} gives the average channel power of the system, which can be used to normalize the average power.


Next, an alternate characterization of GGCs is in terms of gamma distributions is noted. Recall that the gamma density with shape parameter $\alpha$ and rate parameter $\theta$ (represented as $Gamma(\alpha,\theta)$) is given by 
\begin{align}
\label{eqn:gammaPDF}
\pdf{X}{x}=\frac{x^{\alpha-1}\theta^{\alpha}}{\Gamma(\alpha) } \exp\left(-\theta x \right) \;,
\end{align}
where $\Gamma(\cdot)$ is the Gamma function. Then, an arbitrary GGC is a weak limit of a sequence of convolutions of gamma distributions with suitably chosen parameters. For a nondegenerate GGC, the Thorin measure $\mu$ evaluated in the interval $[u,u+\D u)$ represents the shape parameter of a Gamma distribution with rate $u$ which is part of the convolution of Gamma distributions yielding the GGC. It is straightforward to see that, if $X_{1}$ and $X_{2}$ are two GGCs with Thorin measures $\mu_{1}$ and $\mu_{2}$, then $X_{1}+X_{2}$ is a GGC with a Thorin measure $\mu_{1}+\mu_{2}$.  

We now summarize some useful properties of non-degenerate GGCs. 

The density of a GGC with finite Thorin mass exists, and can be written in terms of {\cm} functions as follows:
\begin{lem}
\label{prop:GGC_density}{{\cite[Theorem 4.1.1, Theorem 4.1.2]{book:bondessonGGC}}}
The density of a GGC with Thorin mass $\alpha < \infty$ can be written in the form 
\begin{align}
\label{eqn:GGCPDF_canonical}
\pdf{X}{x} = x^{\alpha -1}h(x) \;,
\end{align}
where $h(\cdot)$ is a c.m. function, which is slowly varying at $0$. Moreover, $h(0+)$ is finite if and only if $\int_{1}^{\infty} \log u \mu(\D u) < \infty$, and in this case 
\begin{align}
\label{eqn:hofzero}
h(0+) = \frac{1}{\Gamma(\alpha)} \exp\left( \int\limits_{0}^{\infty} \log u \mu(\D u) \right) \;.
\end{align}
\end{lem}
The representation of the PDF of a GGC in the form \eqref{eqn:GGCPDF_canonical} is particularly interesting from a wireless system point of view, because $\alpha$ corresponds to the diversity order, and $h(\rho^{-1})$ is directly proportional to the array gain, as shown in Section \ref{sec:GGCasympSER}. GGCs are also mixtures of Gamma distributions, as summarized in the following Lemma:
\begin{lem}{{\cite[Theorem 4.1.1]{book:bondessonGGC}}}
\label{lem:GGC_gammaMixture}
If $X$ is a GGC with Thorin mass $\alpha < \infty$, then $X = A Z$, where $Z \sim Gamma(\alpha,1)$ and $A \geq 0$ are independent. Moreover, $h(x)$ in \eqref{eqn:GGCPDF_canonical} is given by 
\begin{align}
\label{eqn:GGCGammahxandA}
h(x) = (\Gamma(\alpha))^{-1}\E{}{A^{-\alpha}\exp(-x/A)}\;.
\end{align}
\end{lem}
Interpreting $X$ as the instantaneous {\effch} of a GGC channel, from Lemma \ref{lem:GGC_gammaMixture} it is straightforward to see that every GGC channel with finite diversity order is equivalent to a variance mixture of a Nakagami-$m$ channel. This is because the instantaneous {\effch} corresponding to Nakagami-$m$ fading is Gamma distributed \cite{tega04}. We will show in Section \ref{sec:GGCandHCMChannels} that several fading distributions such as Nakagami-$m$, Pareto and generalized gamma distributions have instantaneous {\effch}s which are GGC RVs with finite Thorin diversity order.     
%
%Examples of distributions in $\GGC$ are the Gamma distribution, the Pareto distribution, the Weibull distribution, the inverse Gamma distribution, the positive skewed stable distribution with MGF $\exp(-s^{\alpha})$ where $\alpha \geq 0$, and the lognormal distribution. 
\subsubsection{Hyperbolically Completely Monotone RVs}
A subset of $\GGC$, consisting of the distributions for which the density is a hyperbolically completely monotone (HCM) function is denoted by $\HCM$, and the RVs corresponding to distributions in this set are called HCM RVs. We recall that a function $g$ is defined to be a HCM function if $g(uv)g(u/v)$ can be written as \cite[p. 68]{book:bondessonGGC}
\begin{align}
g(uv)g(u/v) = \int\limits_{0}^{\infty}\exp(-\lambda u (v+v^{-1}))K(\D u ; u)\;, K(\D u ; u) \geq 0\;,
\end{align}
for each $u>0$. HCM RVs enjoy the following properties under products and quotients of RVs, which will be useful in obtaining closure results for wireless systems involving multiple fading RVs:
\begin{lem}
\label{lem:props_GGC_HCM}
If $X_{1}, X_{2}$ are independent HCM RVs, and $Y$ is a GGC independent of $X_{1}$ and $X_{2}$, then
\begin{enumerate}[(i)]
\item $X_{1}^{q} \in  \HCM$, for $|q| \geq 1$.
\item $X_{1}X_{2} \in \HCM$.
\item $X_{1} Y \in \GGC$.
\end{enumerate}
\end{lem} 

The density of a HCM RV admits the following canonical characterization
\begin{lem}{{\cite[p.~81]{book:bondessonGGC}}}
\label{lem:HCMpdf}
The density function of a HCM RV admits the canonical form 
\begin{align}
\label{eqn:hcm_canonicalPdf}
\pdf{X}{x} = C x^{\alpha -1} p_{1}(x) p_{2}(1/x)\;
\end{align}
where $\alpha \in \re$, and
\begin{align}
p_{j}(x) = \exp\left( -b_{j} x -\int\limits_{0}^{\infty}\log\left( \frac{x+y}{1+y}\right)T_{j}(\D y)\right)\;,
\end{align}
with $b_{j} \geq 0$, and $T_{j}(\D y)$ being non-negative measures on $(0,\infty)$ satisfying $\int_{0}^{\infty} (1+y)^{-1}T_{j}(\D y) < \infty$, $j=1,2$.
\end{lem}
In the case of HCM RVs, the Thorin mass can be represented in terms of the parameters $\alpha, b_{j}$ and $T_{j}$ as 
\begin{lem}{{\cite[p.~74]{book:bondessonGGC}}}
\label{lem:HCMthorinMass}
If $X$ is  a HCM RV with canonical PDF parameters $\alpha, b_{j}$ and $T_{j}$, $j=1,2$, then 
\begin{align}
\label{eqn:HCM_thorin_mass}
\int_{0}^{\infty} \mu(\D s) = \begin{cases}
\alpha + T_{2}([1,\infty])&, \mathrm{if}\; b_{2} = 0 \\
\infty &, \mathrm{if}\; b_{2} \neq 0
\end{cases} \;.
\end{align}
\end{lem}
Many RVs relevant to wireless communications are HCM RVs. For example, the Gamma RV, the positive stable RV and the lognormal RV are HCM RVs. In this work, we require the conditions under which the Thorin mass of a sum or product of GGC's is finite. To the best of our knowledge, these conditions were not found elsewhere in the literature, although it is not too difficult to derive them.
\begin{proposition}
\label{prop:ggcCombFiniteThorinMass}
Let $X_{1}, X_{2}, X_{3}$ be independent nonnegative RVs, where $X_{1}$ and $X_{2}$ are GGC's and $X_{3}$ is a HCM RV. Then
\begin{enumerate}[(i)]
\item The Thorin mass of $X_{1}+X_{2}$ is finite if and only if the Thorin masses of both $X_{1}$ and $X_{2}$ are finite.
\item The Thorin mass of $X_{1}X_{3}$ is finite if the Thorin mass of either $X_{1}$ or $X_{3}$ is finite.
\item The Thorin mass of $X_{3}^{-1}$ is finite if the canonical parameters of $X_{3}$ in \eqref{eqn:hcm_canonicalPdf} satisfy $\alpha < \infty$, $b_{1} = 0$ and $T_{1}([1,\infty))< \infty$.
\end{enumerate}
\end{proposition}

%\subsubsection{Extended Generalized Gamma Convolutions}
%An extension of $\GGC$ to a class of distributions on $\re$ is the set of extended GGCs (EGGC), denoted by $\EGGC$. A distribution belongs to $\EGGC$ if the RV is the limit of a sequence of sums of positive and negative Gammma RVs with suitable chosen parameters. Examples of such RVs are the Gaussian distribution, the Symmetric alpha-stable distribution and the set of all distributions in $\GGC$. Symmetric EGGCs are closely related with GGC due to a characterization theorem: A RV $X$ is a symmetric EGGC if and only if can be written as $\sqrt{A}Z$, where $Z \sim \mathcal{N}(0,1)$, and $A$ is a GGC independent of $Z$. EGGCs are closed under scaling, additions and subtractions of RVs.
%
%Similar to EGGC, an extension of HCM RVs has been proposed in the literature. A RV is an extended HCM (EHCM) RV, if and only if it can be written as $\sqrt{A}Z$, where $Z \sim \mathcal{N}(0,1)$ and $A$ is a HCM RV independent of $Z$. Some useful properties of EHCM and EGGC RVs are as follows:
%\begin{itemize}
%\item If $X$ is an EGGC (EHCM), then $X^{2}$ is a GGC (HCM) RV.
%\item If $X_{1}$ and $X_{2}$ are EHCM RVs, then $X_{1}X_{2}$ and $X_{1}/X_{2}$ are both EHCM RVs.
%\item If $X_{1}$ is an EGGC RV, and $X_{2}$ is an EHCM RV, then $X_{1}X_{2}$ and $X_{1}/X_{2}$ are both EGGC RVs. 
%\end{itemize}
\subsection{Stochastic Ordering}
\label{sec:StochPreliminaries}
Stochastic orders are binary relations among RVs, which are used to compare one RV with respect to another. A systematic development of stochastic ordering theory can be found in \cite{shakedbook94}. We now summarize some existing stochastic orders relevant to this paper.
%\subsubsection{Usual Stochastic Order}
% The usual stochastic order compares the magnitude of two RVs, and is equivalent to comparing the CDFs of the RVs. Formally, if the CDF of RV $X$ is $\CDF{X}{\cdot}$, and similarly for RV $Y$, then we write 
%\begin{equation}
%\label{eqn:usual_stochastic_defn}
%X \orderl{st} Y \iff \CDF{X}{x} \geq \CDF{Y}{x} \; \forall x \;.
%\end{equation}
%It is possible to show that $X \orderl{st} Y$ if and only if $\E{}{g(X)} \leq \E{}{g(Y)}$ for all non decreasing functions $g$.
%{\parspadj}
%\subsubsection{Increasing Concave Order}
%Let $X$ and $Y$ be two RVs. Then $X$ is said to be increasing concave ordered with $Y$ (denoted $X \orderl{icv} Y$) if $\E{}{g(X)} \leq \E{}{g(Y)}$ for all non-decreasing concave functions $g$, such that the expectations exist. A necessary and sufficient condition for the $\orderl{icv}$ order to hold \cite{shakedbook94} is the following:
%\begin{align}
%   \label{eqn:cx_cond1}
%     X \orderl{icv} Y \iff \int\limits_{- \infty}^{x}  \CDF{X}{u} \D u  \geq \int\limits_{- \infty}^{x}  \CDF{Y}{u} \D u \;, \forall x \;.
%\end{align}
%It is easy to see that by choosing $g(x) = x$, which is non-decreasing and concave, we obtain
%\begin{align}
%\label{eqn:icv_expectation}
%X \orderl{icv} Y \implies \E{}{X} \leq \E{}{Y} \;,
%\end{align}
%whenever the expectations exist.
%
%The $\orderl{icv}$ order can be interpreted from a wireless communications perspective. Let $\rho \geq 0$ be the average SNR, and $\rho X$, $\rho Y$ represent the instantaneous SNRs of two fading distributions. Then the $\orderl{icv}$ order can be used to compare the ergodic capacities of the two fading channels, since the instantaneous capacity function $g(x) = \log(1+\rho x)$ is an increasing and concave function.
\subsubsection{Laplace Transform Order}
\label{subsec:LTorder}
Similar to $\orderl{icv}$, it is possible to order {\rv}s based on their Laplace transforms (LT). The LT order is defined as follows:
\begin{align}
\label{eqn:LT_expectations}
X \orderl{Lt} Y \iff \E{}{\exp(-\rho Y )} \leq \E{}{\exp(-\rho X )}  \forall \; \rho > 0 \; .
\end{align}
This order is interesting from the context of the current paper, because the LT of a GGC RV is of the form $\exp (-\gamma(s))$, where $\gamma$ is a {\tbf}. As a result, LT ordering of GGC RVs corresponds to pointwise ordering of {\tbf}s. One of the powerful consequences of LT ordering is the following: 
\begin{align}
\label{ch2:eqn:LT_order_relation}
X \orderl{Lt} Y \iff \E{}{\g(X)} \geq \E{}{\g(Y)} \; ,
\end{align}
for all \emph{completely monotonic} ({\cm}) functions $g(\cdot)$ \cite[pp. 96]{shakedbook94}. A similar result with a reversal in the inequality states that 
\begin{align}
\label{ch2:eqn:LT_order_relation_1}
X \orderl{Lt} Y \iff \E{}{\g(X)} \leq \E{}{\g(Y)} \;,
\end{align}
for all Bernstein functions $\g(\cdot)$. In addition, we know that
\begin{align}
\label{ch2:eqn:LT_order_relation_2}
X \orderl{Lt} Y \iff \g(X) \orderl{Lt} g(Y)\;,
\end{align}
for all Bernstein functions $\g(\cdot)$.

Another useful result for Laplace transform ordered RVs is the following:
\begin{lem}
\label{prelims:LT_MultivariateFn}
Let $X_{1},\ldots,X_{M}$ be independent and $Y_{1},\ldots,Y_{M}$ be independent. If $X_{m} \orderl{Lt} Y_{m} , \;  m = 1,\ldots,M$, then $g\left(X_{1},\ldots,X_{M}\right) \orderl{Lt} g\left(Y_{1},\ldots,Y_{M}\right)$, if $g(x_{1},\ldots,x_{M})$ is a Bernstein function of $x_{i}$, when all other arguments of $g$ are viewed as constants.
\end{lem}

In a wireless communications context, let $\rho \geq 0$ be the average SNR, and $\rho X$, $\rho Y$ represent the instantaneous SNRs of two fading distributions. If $g(x)$ corresponds to the instantaneous SER $P_{\mathrm{ e}}(\rho x)$ of a modulation scheme such as MPSK whose SER is a {\cm} function \cite{paper:adithyaSER}, then \eqref{ch2:eqn:LT_order_relation} can be used to obtain comparisons of averages of SERs over pairs of fading channels, even in cases where a closed-form expression for the same is intractable. 

%\subsubsection{Ergodic Capacity Order}
%Another stochastic order which we will use in this work, is the ergodic capacity order, introduced in \cite{paper:adithyaCapacityconf}. Let $X$ and $Y$ be two nonnegative RVs such that $\E{}{\log(1+\rho X)}< \infty$ and $\E{}{\log(1+\rho Y)} < \infty $. Then $X$ is said to be dominated by $Y$ in the ergodic capacity sense (denoted as $X \orderl{c} Y$) if $\E{}{\log(1+\rho X)} \leq \E{}{\log(1+\rho Y)}$, for $\rho \geq 0$. 
%The ergodic capacity order and the LT order are related as follows:
%\begin{lemma}{{\cite[Property S3]{paper:capacityArxiv}}}
%\label{lem:GGCLTimpCap}
%Let $X$ and $Y$ be two nonnegative RVs. Then $X \orderl{Lt} Y \implies X \orderl{c} Y$. However it is not true in general that $X \orderl{c} Y \implies X \orderl{Lt} Y$.
%\end{lemma}
%Intuitively, while the LT order between two instantaneous {\effch} RVs can be viewed as the ordering of the two fading channels based on the ergodic capacity and error rate metrics, the ergodic capacity ordering between the two RVs implies that although the channels are ordered based on the the ergodic capacity, they need not be ordered with respect to the error rate at all SNR.

%Although the LT order is useful in applications such as the ordering GGC RVs, it are not applicable when we consider the problem of the ordering the Laplace exponents of GGCs. 

This is because the above mentioned stochastic orders 

As a result, we need to define generalizations of the LT order and the ergodic capacity order, which cater to cases when the measures need not integrate to unity.
\subsubsection{Generalized Shannon Transform Order and Generalized LT order}
In what follows, we propose two new stochastic orders between two non-negative measures, which are generalizations of the ergodic capacity order proposed in \cite{paper:adithyaCapacityconf} and the LT order. We need these generalizations, because the ergodic capacity order and the LT order are based on comparisons of transforms (Shannon transform and LT) of measures which integrate to unity, such as the densities of RVs. The applications we consider in this work  do not necessarily involve measures integrating to unity. 

Let $\mu$ be a non-negative measure. We define its generalized Shannon transform as $\int_{0}^{\infty} \log (1+s/u) \mu (\D u)$. If $\mu_{1}$ and $\mu_{2}$ are two non-negative measures for which the generalized Shannon transforms exist and are finite, then we say $\mu_{1}$ is dominated by $\mu_{2}$ in the generalized Shannon transform sense, and write $\mu_{1} \orderl{gS} \mu_{2}$ to denote $\int_{0}^{\infty} \log(1+s/u) \mu_{1} (\D u)  \leq \int_{0}^{\infty} \log (1+s/u) \mu_{2} (\D u)$, for all $s \geq 0$. 
Similarly, $\mu_{1}$ is said to be dominated by $\mu_{2}$ in the generalized Laplace transform sense (denoted by $\mu_{1} \orderl{gLt} \mu_{2}$ if $\int_{0}^{\infty} \exp(-s u) \mu_{1}(\D u) \geq \int_{0}^{\infty} \exp(-s u) \mu_{2}(\D u)$, for all $s \geq 0$.

Some properties of the generalized Shannon transform order and the Generalized LT orders are the following:\\
\textbf{P1}: If $\int_{0}^{\infty}\mu_{1}(\D u) = \int_{0}^{\infty}\mu_{2}(\D u) < \infty$, then $\mu_{1} \orderl{gLt} \mu_{2} \implies \mu_{1} \orderl{gS} \mu_{2}$\\
\textbf{P2}: $\mu_{1} \orderl{gS} \mu_{2} \iff \int_{0}^{\infty} \sigma (u) \mu_{1}(\D u)  \leq \int_{0}^{\infty} \sigma (u) \mu_{2}(\D u)  $, for all $\lbrace \sigma \in \TBF | \sigma(0) = 0 \rbrace$.\\
\textbf{P3}: Let $\int_{0}^{\infty} \mu_{1}(\D u) \leq \int_{0}^{\infty} \mu_{2}(\D u)$. Then $\mu_{1} \orderl{gS} \mu_{2} \iff \int_{0}^{\infty}  \sigma (u) \mu_{1}(\D u) \leq \int_{0}^{\infty} \sigma (u) \mu_{2}(\D u) $, for all $\sigma \in \TBF$.
\section{A Unified Fading Model using GGCs}
\label{sec:GGCandHCMChannels}
In this work, we propose to view instantaneous {\effch} distributions as members of $\GGC$. Hereafter, we refer to channels with GGC distributed {\effch} as GGC channels. To justify that the $\GGC$ class is indeed a unification of fading distributions, we show that many of the popularly used fading channels are GGC channels. Among the GGC channels, we identify distributions for which the instantaneous {\effch} is a HCM RV, as this fact will be useful in the analysis of systems, where the overall instantaneous {\effch} RV involves a product of two or more RVs (See Section \ref{sec:GGCPerfBoundsSys}). We now give explicit examples of RVs belonging to $\GGC$ and $\HCM$.

%To begin with, we give an example of a typical wireless system which turns out to be a GGC channel.
%\begin{example}
%\label{prop:prop_h_X}
%Consider the channel model $y = \sqrt{\rho} h s + v$, where $v$ is a standard Gaussian RV, $\rho \geq 0$ represents the average SNR, $s$ is the transmitted symbol, $h = \sqrt{A}(z^{\mathrm{R}}+ j z^{\mathrm{I}})$, with $\CDF{A}{\cdot} \in \GGC$, $z^{\mathrm{R}}$ and $z^{\mathrm{I}}$ are standard Gaussian RVs, and all the RVs are independent of each other. Then the instantaneous channel power distribution is a GGC.
%\end{example}
%\begin{IEEEproof}
%Observe that $X = |h|^{2} = AE$, where $E$ is exponentially distributed. We will show in Section \ref{sec:GammaDistGGC} that the exponential distribution belongs to $\HCM$. Since $A$ is assumed to be a GGC, from Lemma \ref{lem:props_GGC_HCM} it follows that $AE$ is a GGC.
%\end{IEEEproof}
%From Example \ref{prop:prop_h_X}, one sees that a sufficient condition for a fading channel to be a GGC is that the real and imaginary parts of the fading are Gaussian mixtures. Alternatively, if $A$ is viewed as a multiplicative RV which captures the long-term fluctuation of the variance of the complex fading process (referred to as shadowing), then Example \ref{prop:prop_h_X} suggests that a Rayleigh fading channel with GGC shadow fading is equivalent to a GGC fading channel.
%First, we note from Lemma \ref{lem:GGC_gammaMixture} that a GGC instantaneous {\effch} distribution with finite Thorin mass corresponds to the product of an independent Gamma RV and a non-negative RV. Therefore, regardless of the empirical basis of the fading model, we discover that any such distribution is a composite shadowing and Nakagami-$m$ fading model, because the instantaneous power of a Nakagami-$m$ channel is Gamma distributed. Alternatively, the GGC unification shows that any GGC fading effect can be viewed as the resultant effect of contributions from infinitely many independent Nakagami-$m$ channels. Specifically, if the received power in a wireless network is a result of many (possibly infinite) coherently combined independent paths which undergo Nakagami-$m$ fading with different $m$ parameters, then the overall fading effect is equivalent to a GGC fading channel.
%To establish that a given channel is a GGC channel, we need to show that its Laplace exponent is a Thorin-Bernstein function. Alternatively, it is easier to show that some fading distributions are GGCs, by showing that they are HCM.

%In order to justify this claim, we must at least ensure that known shadowing distributions are members of this class. Toward this end, we show that several shadowing distributions used in the literature, such as lognormal \cite[p. 23]{simon_alouini05}, gamma \cite{paper:alouini} and inverse Gaussian \cite{gopal2012performance} in fact belong to $\HCM$. We therefore propose to view shadowing distributions as members of $\HCM$, and in doing so we are able to exploit the additional properties satisfied by HCM RVs. 

%To establish that a given channel is a GGC channel, we need to show that its Laplace exponent is a Thorin-Bernstein function. Alternatively, it is easier to show that some fading distributions are GGCs, by showing that they are HCM.
%\subsubsection{Exponential Distribution}
%The distribution of an exponential RV is given by $\pdf{X}{x} = \exp(-x)$, and the corresponding MGF is $\MGF{X}{s} = (1+s)^{-1}$. It is easily shown that the Thorin measure is given by
%\begin{align}
%\label{eqn:exp_thorinMeasure}
%\mu(u) = \delta(u-1)\;,
%\end{align}
%where $\delta(\cdot)$ is the Dirac delta function. Consequently, the Thorin mass is obtained to be $\alpha = 1$. It is also a HCM RV, with parameters $\beta=1$, $b_{1} = 1$, $b_{2}=0$, $\Gamma_{j} = 0$, $j=1,2$. The exponential distribution arises as the instantaneous channel power distribution in Rayleigh fading channels.
\subsection{Gamma Distribution}
\label{sec:GammaDistGGC}
The Gamma distribution defined by \eqref{eqn:gammaPDF} with parameters $k$ and $\theta$ has LT given by $\MGF{X}{s} = \exp(-k \log(1+s/\theta))$, which satisfies the representation of the LT of a GGC specified in \eqref{eqn:MGF_GGC_gen}. It is then straightforward to show using \eqref{eqn:MGF_GGC_gen} that the Thorin measure in this case, is given by
\begin{align}
\label{eqn:gammaThorinMeas}
\mu(u) = k \delta(u-\theta)\;,
\end{align}
and the Thorin mass is $k$, as can be verified by rewriting the PDF in the form \eqref{eqn:GGCPDF_canonical}. Further if $k < \infty$, then $h(\cdot)$ is given by $h(x) = \theta \exp(-\theta x)/\Gamma(k)$. The gamma distribution also belongs to $\HCM$, with canonical parameters of \eqref{eqn:hcm_canonicalPdf} specified by $\alpha=k$,  $b_{1} = \theta$, $b_{2}=0$, $T_{j} = 0, j=1,2$.

Gamma RVs with $\theta = k$ correspond to the instantaneous {\effch} of Nakagami-$m$ fading  \cite{tega04}, and are used to model short-term fading effects in line of sight channels. The Gamma distribution has also been used to model long-term fading effects in the literature \cite{alouini1999unified}. Moreover, the exponential distribution, which is a special case of a Gamma RV with $k=\theta=1$ arises as the instantaneous fading power distribution in Rayleigh fading channels. 
\subsection{General Lognormal Distribution}
The density of the general lognormal RV is given by
\begin{align}
\label{eqn:logNormalPDF}
\pdf{X}{x} = c x^{\mu/\sigma^{2} -1}\exp\left( -\frac{(\log x)^{2}}{2 \sigma^{2}}\right)\;,
\end{align}
with $\mu \in \re, \sigma >0$. It has been shown in \cite[p.~74]{book:bondessonGGC} that the general lognormal distribution belongs to $\HCM$, and hence also $\GGC$. Although the Thorin measure is unknown, the canonical parameters of \eqref{eqn:hcm_canonicalPdf} are known to be $b_{1}=b_{2}=0$, $\alpha = \mu/\sigma^{2}$ and $T_{j}(u) = \sigma^{-2} u^{-1}, u>1$ \cite[p.~74]{book:bondessonGGC}, and the Thorin mass can be calculated from \eqref{eqn:HCM_thorin_mass} to be $\infty$. The lognormal distribution is commonly used to model the long-term fading effect in wireless channels \cite{simon_alouini05}.
\subsection{Generalized Gamma Distribution}
The density corresponding to the generalized gamma distribution is given by 
\begin{align}
\label{eqn:GenGammDist}
\pdf{X}{x} = c_{1} x^{\epsilon -1} \exp\left( -c_{2} x^{r}\right)\;,
\end{align}  
where $0 < |r| \leq 1$, $c_{1},c_{2} \geq 0$, and $\epsilon /r >0$. To see that this distribution belongs to $\GGC$, we will show that it is HCM, and therefore GGC. To this end, it is known that if $X$ is a generalized Gamma distributed RV with PDF given by \eqref{eqn:GenGammDist}, then 
\begin{align}
\label{eqn:GenGammaAndGamma}
X=Y^{1/r}\;, 
\end{align}
where $Y \sim Gamma(\epsilon/r,c_{2})$. Since the Gamma distribution belongs to $\HCM$, as shown in Section \ref{sec:GammaDistGGC}, it follows from Lemma \ref{lem:props_GGC_HCM} that the generalized gamma distribution also belongs to $\HCM$, and is therefore a GGC. While the Thorin measure for the general case is unknown, the Thorin mass is equal to $\epsilon$ if $r>0$, and $\infty$ otherwise, as can be verified by representing \eqref{eqn:GenGammDist} in the form \eqref{eqn:GGCPDF_canonical}, and further, the function $h(\cdot)$ is given by $h(x) = c_{1}\exp(-c_{2}x^{r})$. 

In a wireless communications context, it can be shown through \eqref{eqn:GenGammaAndGamma} that the generalized gamma distribution arises as the instantaneous {\effch} distribution in Nakagami-$m$ fading channels with receiver non-linearity, where the non-linearity is captured as a power parameter. In addition, the distribution of the instantaneous {\effch} is generalized Gamma distributed, when the envelope of the fading amplitude is modelled as a generalized Nakagami-$m$ RV \cite{alouini1999unified}. Moreover, the Weibull distribution is a special case of the density in \eqref{eqn:GenGammDist}, which has been used to approximate the multipath wireless channel from channel measurements \cite{sagias2004channel}. Other distributions which are special cases of the generalized Gamma distribution are the inverse-Gaussian distribution and the Nakagami-$m$ distribution.
\subsection{Product of Generalized Gamma Random Variables}
Consider $X$ to be a product of $N$ independent but not necessarily identically distributed generalized Gamma distributed RVs. This distribution is HCM as observed from an application of Lemma \ref{lem:props_GGC_HCM} and the fact that the generalized Gamma distribution belongs to $\HCM$. 

We make special mention of this distribution, as it has been proposed as a unified fading model in the literature \cite{sagias2006performance}. In addition, as a special case, we get a product of $N$ independent Gamma RVs, which is the instantaneous channel power distribution in the $N*$Nakagami fading model, where the envelope is  a product of $N$ independent but not necessarily identically distributed Nakagami-$m$ RVs \cite{paper:Nstarnakagami, andersen2002statistical}.
\subsection{Positive Stable Distribution}
The positively skewed stable distribution is a heavy tailed distribution, which is characterized by its LT as $\MGF{X}{s} = \exp(-s^{r})$, $0<r \leq 1$. No closed form expression for the distribution or density is known in general. Nevertheless, it is known that this distribution is a GGC \cite[p. 35]{book:bondessonGGC}, with Thorin measure given by 
\begin{align}
\label{eqn:posStableThorinMeas}
\mu(u) =\frac{r \sin r \pi}{\pi}u^{r-1}\;,
\end{align}
and Thorin mass equal to $\infty$. It has been established in the literature that this distribution belongs to $\HCM$ when $r$ is the inverse of a positive integer \cite[p. 85]{book:bondessonGGC}. 

Positive stable distributions have been used to model the interference at the primary receiver in a cognitive radio network, when the interfering secondary terminals are distributed in a Poisson field, and there is a guard zone around the primary receiver \cite{hong2008interference}.
\subsection{Pareto Distribution}
The Pareto distribution given by the density
\begin{align}
\label{eqn:ParetoPDF}
\pdf{X}{x} = \frac{|r|}{B(k_{2},k_{1})}\frac{x^{k_{1}r-1}}{(1+x^{r})^{k_{1}+k_{2}}}\;,
\end{align} 
where $B(a,b) := \int_{0}^{1} t^{a-1}(1-t)^{b-1} \D t$ is the Beta function, $r \in [-1,1]$, $k_j > 0$, $j=1,2$. The Pareto distribution belongs to $\HCM$, as a Pareto RV can be written in the form \cite[p. 14]{book:bondessonGGC}
\begin{align}
\label{eqn:paretoIsGammaRatio}
X = \left(\frac{X_{1}}{X_{2}} \right)^{\frac{1}{r}}\;,
\end{align}
where $X_{j} \sim Gamma(k_{j},1)$, $j=1,2$. Since Gamma RVs are HCM, from Lemma \ref{lem:props_GGC_HCM} it follows that a Pareto RV is HCM. The Thorin measure is unknown in the general case, however the Thorin mass is obtained from Lemma \ref{lem:HCMthorinMass} as $k_{1} r$. 

The fact that Pareto RVs are ratios of Gamma RVs raised to a non-negative power, as shown in \eqref{eqn:paretoIsGammaRatio} leads to many wireless systems with Pareto instantaneous {\effch}. For example, consider a system with a transmitter, receiver and an interfering terminal. Suppose the channel between the transmitter and the receiver, and that between the interferer and receiver are both Nakagami-$m$ channels (with not necessarily identical parameters), and the receiver is non-linear with the non-linearity captured in the form of a power parameter. Then from \eqref{eqn:paretoIsGammaRatio}, it is clear that the instantaneous {\effch} is a Pareto RV. We also note that special cases of the Pareto distribution with $(k_{1}=k_{2}=1, r>0)$ have been used to model the instantaneous signal to interference power in interference dominated networks \cite{pun07}.
\section{Performance Metrics for GGC Channels}
In this Section, we obtain expressions for the performance metrics of GGC channels in terms of the Thorin measure and/or the function $h(\cdot)$ defined in \eqref{eqn:GGCPDF_canonical}, which characterize the GGC.
\label{sec:GGC_performanceMetrics}
\subsection{Ergodic Capacity}
The ergodic capacity $\Cerg{X}{}$ of a fading channel is defined as the maximum rate at which information may be transmitted over the channel, when there is channel side information at the receiver only, and coding at the transmitter may be applied across multiple realizations of the channel. In this case, it is well known that $\Cerg{X}{} = \E{}{\log(1+\rho X)}$, where $X$ is the instantaneous {\effch}. We will now see that when $X$ is a GGC, its Thorin measure can be used to determine the ergodic capacity.
\begin{proposition}
Let $\gamma(\cdot)$ be the Laplace exponent of a GGC $X$. Then
\begin{align}
\label{eqn:GGC_cerg_full}
\Cerg{X}{} = \int\limits_{0}^{\infty}\frac{\exp(-s)}{s}\left( 1 - \exp(-\gamma(\rho s )) \right) \D s \;.
\end{align}
\end{proposition}
Since $\gamma(\cdot)$ is determined by the Thorin measure, we conclude that the ergodic capacity is a function of the Thorin measure.
\subsection{Average Symbol Error Rate}
Consider the following system model
\begin{align}
\label{eqn:GGC_sysmodel_pe}
y = \sqrt{\rho X}s + w\;,
\end{align}
where $\rho \geq 0$ is the average SNR, $w$ is circularly symmetric AWGN, and $X$ is the instantaneous {\effch}, whose distribution belongs to $\GGC$. We obtain the average SER $\AvgPe{}{\cdot}$ for the case when the transmitted symbol $s$ belongs to an MPSK constellation, and also for the case when it belongs to an MQAM constellation. In both these cases, the instantaneous SER (i.e., SER conditioned on $X=x$) is known to be a function of the form $P_{\mathrm{e}}(\rho x) = \int_{0}^{\infty} \exp(-\rho x u) \eta(u) \D u$, where $\eta(\cdot)$ is a nonnegative function which depends on the constellation \cite {paper:adithyaSER}. Specifically, for MPSK, $\eta(u) = (\sin (\pi/M)/(2 \pi))I[u \geq 1]/(u\sqrt{u-\sin^{2}(\pi/M)})$.
\begin{proposition}
\label{prop:GGC_fullSER}
For the system model \eqref{eqn:GGC_sysmodel_pe}, 
\begin{align}
\AvgPe{}{\rho} = \int\limits_{0}^{\infty}\exp\left( -\gamma(\rho u)\right) \eta(u) \D u\;,
\end{align}
where $\gamma(\cdot)$ is the Laplace exponent of the GGC, and $\eta(u)$ depends on the constellation.
\end{proposition}
According to Proposition \ref{prop:GGC_fullSER}, if the modulation scheme is fixed as MPSK or MQAM, then the average SER depends only on the Laplace exponent, which in turn depends only on the Thorin measure of the GGC.
\subsubsection{Asymptotic Symbol Error Rate}
\label{sec:GGCasympSER}
We now analyze the average SER performance of a channel with GGC instantaneous fading power at high SNR. As we will see, the asymptotic SER will be represented in terms of the Thorin measure of the GGC. To begin with, we establish a necessary and sufficient condition under which the average SER $\AvgPe{}{\cdot}$ is linear in a log-log scale at high SNR, because our aim is to obtain the high SNR SER expression in terms of the diversity order of system, which is relevant only if $\AvgPe{}{\cdot}$ satisfies this condition.
%\begin{theorem}
%\label{thm:GGCSER_Linear}
%Consider a GGC fading channel with instantaneous fading power $X$, and let its Thorin measure be $\mu$. If $\int_{0}^{\infty} u^{n} \mu(u) \D u < \infty,\; \forall n \in \lbrace 0,1,2,\ldots \rbrace$, then $\AvgPe{}{\cdot} = (G \rho)^{-D} + O(\rho^{-D-1})$ as $\rho \rightarrow \infty$, where $G >0$ and $0<D<\infty$. Conversely, if $\int_{0}^{\infty} u^{n} \mu(u) \D u = \infty$ for some $n \in \lbrace 0,1,2,\ldots \rbrace$, then $\AvgPe{}{\rho}$ decays more rapidly than a linear function on a log-log scale as $\rho \rightarrow \infty$.
%\end{theorem} 
%
%Although Theorem \ref{thm:GGCSER_Linear} is a necessary and sufficient condition to establish the liearity of the average SER at high SNR on a log-log scale, it can sometimes be tedious or impossible to determine if a given GGC satisfies the conditions required by Theorem \ref{thm:GGCSER_Linear}. Therefore, we derive a simpler sufficient condition based on Theorem \ref{thm:GGCSER_Linear}.
%\begin{corollary}
%\label{corr:GGClinearsuff}
%Consider a GGC fading channel with instantaneous fading power $X$, and let its Thorin measure be $\mu$. If $\mu(u)$ is continuous, with $\mu(u) = O(u^{-1}), u \rightarrow 0+$ and $\mu(u) = 0 , u > u_{0}$ for some $u_{0} \in \re^{+}$, then $\AvgPe{}{\rho} = (G \rho)^{-D} + O(\rho^{-D-1})$, where $G \in (0,\infty), D \in (0,\infty)$.
%\end{corollary}
%\begin{IEEEproof}
%We prove this corollary by establishing a sufficient condition for 
%\begin{align}
%\label{eqnGGCSER_linearsuf1}
%\int_{0}^{\infty} u^{n} \mu(u) \D u < \infty\;, 
%\end{align}
%for all $n \in \lbrace 0,1,2,\ldots \rbrace$. To this end, we find the condition under which \eqref{eqnGGCSER_linearsuf1} is finite for every $n \in \re^{+}$, which is a stricter requirement than that listed in Theorem \ref{thm:GGCSER_Linear}. This modified criterion is in fact equivalent to the convergence of the Mellin transform of $\mu$ for $n\geq 1$. A sufficient condition to ensure this convergence is the continuity of $\mu$ and $\mu(u) = O(u^{-1}), u \rightarrow 0+$ and $\mu(u) = 0 , u > u_{0}$ for some $u_{0} \in \re^{+}$. Therefore, if $\mu$ satisfies the aforesaid asymptotics, then according to Theorem \ref{thm:GGCSER_Linear}, $\AvgPe{}{\rho} = (G \rho)^{-D} + O(\rho^{-D-1})$, where $G \in (0,\infty), D \in (0,\infty)$.
%\end{IEEEproof}


\begin{proposition}
\label{thm:GGCSER_Linear}
Let a non-degenerate GGC fading channel have Thorin mass $\alpha < \infty$. Then for MPSK/MQAM, we have $\AvgPe{}{\rho} \sim  c_{\mathrm{M}}  h(\rho^{-1}) \rho^{-\alpha}$, as $\rho \rightarrow \infty$, where $c_{\mathrm{M}}$ is depends on the modulation scheme, and $h(\cdot)$ is as defined in \eqref{eqn:GGCPDF_canonical} or \eqref{eqn:GGCGammahxandA}.
\end{proposition} 
\begin{IEEEproof}
According to \cite[Theorem 4]{paper:yuanTauberian}, if the instantaneous {\effch} PDF is of the form $\pdf{X}{x} = D x^{D-1}l(x)$, where $l(x)$ is slowly varying at $0$, then $\AvgPe{}{\rho} \sim c_{\mathrm{M}}\rho^{-D}l(\rho^{-1})$ as $\rho \rightarrow \infty$, if $\AvgPe{}{\rho} \leq a_{1} \exp(-b \rho)$, $a>0, b>0$. To apply this result to our case, we note that MPSK and MQAM have exponentially bounded SERs, as obtained by using the Chernoff bound. Next, we will argue that GGCs with finite Thorin mass satisfy the required condition on the asymptotic PDF. Recall from Lemma \ref{prop:GGC_density} that when the Thorin mass of the GGC is finite, its PDF has the form $x^{\alpha-1}h(x)$, where $h$ is slowly varying at $0$. The proposition is then immediate.
\end{IEEEproof}
The asymptotic SER obtained in Theorem \ref{thm:GGCSER_Linear} applies to any GGC fading channel, and shows that the parameters of the GGC, such as the Thorin mass and the function $h$ from density representation in Lemma \ref{prop:GGC_density} determine the asymptotic SER parameters. For GGC channels satisfying a certain condition on the Thorin measure, we can show that the asymptotic SER is of the form $\AvgPe{}{\rho} \sim \cg{}\rho^{-\alpha}$, as shown in the following Proposition:
\begin{proposition}
\label{prop:GGCasympSERalt}
Let the Thorin measure of a nondegenerate GGC fading channel with finite Thorin mass $\alpha$ satisfy $\int_{1}^{\infty} (\log u) \mu(\D u) < \infty$. Then $\AvgPe{}{\rho} \sim \cg{}\rho^{-\alpha}$, as $\rho \rightarrow \infty$.
\end{proposition}
\begin{proof}
From Proposition \ref{thm:GGCSER_Linear}, we get
\begin{align}
\label{eqn:GGC_asympSERalteqn1}
\lim_{\rho \rightarrow \infty} \frac{c_{\mathrm{M}}^{-1}\rho^{D}\AvgPe{}{\rho}}{h(\rho^{-1}} =1\;.
\end{align}
The limit of the ratio in \eqref{eqn:GGC_asympSERalteqn1} can be written as a ratio of limits of the numerator and denominator, if and only if $\int_{1}^{\infty} (\log u) \mu(\D u) < \infty$, because this is the condition under which $\lim_{\rho \rightarrow \infty}h(\rho^{-1})< \infty$, as can be seen through an application of Lemma \ref{prop:GGC_density}. Therefore, \eqref{eqn:GGC_asympSERalteqn1} simplifies to
\begin{align}
\label{eqn:GGC_asympSERalteqn2}
\lim_{\rho \rightarrow \infty} c_{\mathrm{M}}^{-1}\rho^{D}\AvgPe{}{\rho} = \lim_{\rho \rightarrow \infty} h(\rho^{-1})\;.
\end{align}
The right hand side of \eqref{eqn:GGC_asympSERalteqn1} is given by $\Gamma(\alpha)^{-1}\exp(\int_{0}^{\infty} (\log(u)) \mu(\D u)$, as seen from Lemma \ref{prop:GGC_density}. Substituting this in \eqref{eqn:GGC_asympSERalteqn1} and rearranging, we get
\begin{align}
\label{eqn:GGC_asympSERalteqn3}
\lim_{\rho \rightarrow \infty} \frac{\AvgPe{}{\rho}}{c_{\mathrm{M}}\Gamma(\alpha)^{-1}\exp(\int_{0}^{\infty} (\log(u)) \mu(\D u) \rho^{-D}} =1\;.
\end{align}
This proves the Proposition.
\end{proof}
Thus, we see that for some special cases of GGCs such as Nakagami-$m$, which satisfy  $\int_{1}^{\infty} (\log u) \mu(\D u) < \infty$, the asymptotic SER depends only on the Thorin measure. Moreover, the {\codinggain}, which is defined as the shift of the average SER curve to right, in the plot of average SER versus average SNR, and given by $\cg{}= \lim_{\rho \rightarrow \infty} \rho^{\alpha} \AvgPe{}{\rho}$ can be seen to be
\begin{align}
\cg{} = \frac{c_{\mathrm{M}}}{\Gamma(\alpha)}\exp\left( \int\limits_{0}^{\infty} (\log u) \mu(\D u) \right)\;.
\end{align}
The {\codinggain} will be useful in calculating the performance difference between two GGC fading channels at high SNR, as discussed in Section \ref{sec:GGCperformanceGap}.
%Corollary \ref{corr:GGClinearsuff} shows that the average SER of a Nakagami-$m$ fading channel can be written as $\AvgPe{}{\rho} = (G \rho)^{-D} + O(\rho^{-D-1})$, since its Thorin measure is a delta function, which satisfies $\mu(u) = O(u^{-1}), u \rightarrow 0+$ and $\mu(u) = 0, u > m$. On the other hand, it can be seen from Theorem \ref{thm:GGCSER_Linear} that the average SER of lognormal shadowing channels and systems with positive $\alpha$-stable distributed SIR is nonlinear at high SNR on a log-log scale, because both these distributions satisfy the converse of Theorem \ref{thm:GGCSER_Linear} for $n=0$.
%Theorem \ref{thm:GGCSER_Linear} shows that the asymptotic average SER of a Nakagami-$m$ and Pareto fading channels can be written as $\AvgPe{}{\rho} \sim  c_{\mathrm{M}}  h(\rho^{-1}) \rho^{-\alpha}$, as $\rho \rightarrow \infty$, since the Thorin mass is finite, as shown in Section \ref{sec:GGCandHCMChannels}. 
 
%
%
%On the other hand, it can be seen from Theorem \ref{thm:GGCSER_Linear} that the average SER of lognormal shadowing channels and systems with positive $\alpha$-stable distributed SIR is nonlinear at high SNR on a log-log scale, because both these distributions have infinite Thorin mass.
%\subsubsection{Diversity Order and Array Gain}
%\label{sec:GGCDiversityOrder}
%The diversity order and {\codinggain} are parameters which measure the asymptotic high SNR average SER performance of the fading channel. The diversity order $\DivOrd{X}$ is the log-domain slope of SER in the high SNR regime. On the other hand, the shift of the SER curve to the left is known as the array gain $\cg{X}$. Mathematically, $\DivOrd{X} = -\lim_{\rho \rightarrow \infty} \D \log \AvgPe{}{\rho} / \D \log \rho$, and $\cg{X} = (\lim_{\rho \rightarrow \infty} \rho^{\DivOrd{X}} \AvgPe{}{\rho})^{-1/\DivOrd{X}}$.  In the following discussion, we assume that the modulation scheme employed has a {\cm} SER, because this encompasses several popularly used modulation formats such as DPSK, $M$-PSK and $M$-QAM. In fact, it has been shown in \cite{paper:adithyaSER} that every $1$-dimensional and $2$-dimensional modulation scheme operated over an AWGN channel has a {\cm} SER. A {\cm} SER is by definition bounded by a decreasing exponential function. Under these assumptions, we can now provide expressions for $\DivOrd{X}$ and $\cg{X}$, when $X$ is a GGC which satisfies Theorem \ref{thm:GGCSER_Linear}.
%\begin{theorem}
%\label{thm:DivOrdGGC}
%If the instantaneous channel power $X$ of a fading channel is a GGC, then the diversity order of any modulation scheme with exponentially bounded SER is given by $\DivOrd{X} = \int_{0}^{\infty} \mu(u) \D u$.
%\end{theorem}
%%In other words, if either the left extremity of the GGC is non-zero, or the Thorin mass is infinite, then the diversity order is infinite. A diversity order of infinity indicates that the SER becomes nonlinear on a log-log scale at high SNR. We therefore confine our discussions to GGCs with zero left extremity and finite Thorin mass. 
%
%%Theorem \ref{thm:DivOrdGGC} can be used to obtain the diversity order of a GGC fading channel, if either the Thorin measure or the Thorin mass is known in closed form. However, in cases where these quantities are unknown, the diversity order can still be evaluated from the PDF, if it is known that the instantaneous fading power is HCM. 
%Theorem \ref{thm:DivOrdGGC} can be used to obtain the diversity order of a GGC fading channel, if either the Thorin measure or the Thorin mass is known in closed form. However, in cases where these quantities are unknown, the diversity order can still be evaluated from the PDF represented in the form \eqref{eqn:GGCPDF_canonical}, and is given by $\DivOrd{X} = \alpha$.
%%\begin{theorem}
%%\label{thm:DivOrdHCM}
%%If the instantaneous channel power $X$ of a fading channel is a HCM RV, then the diversity order for a modulation scheme with an exponentially bounded SER is given by 
%%\begin{align}
%%\DivOrd{X} = \beta + \Gamma_{2}([1,\infty])+ b_{2} \infty \;,
%%\end{align}
%%where $\beta, \Gamma_{2}$ and $b_{2}$ are as defined in \eqref{eqn:hcm_canonicalPdf}.
%%\end{theorem}
%%Analogous to the GGC case, we limit our discussions to HCM distributions with $b_{2} < \infty$ and $\Gamma_{2}([1,\infty]) < \infty$, in order to ensure the the system has finite diversity order. 
%Next, we present an expression for the {\codinggain} of a GGC fading channel, which together with Theorem \ref{thm:DivOrdGGC} yields an asymptotic SER expression. The following Theorem applies to any modulation scheme which has a {\cm} SER, such as an arbitrary one-dimensional or two-dimensional constellation \cite{paper:adithyaSER}. In other words, the instantaneous SER is represented as $P_{\mathrm{e}}(\rho X) = \int_{0}^{\infty} \exp(-\rho u X) \eta(u) \D u$, $\rho \geq 0$, where $\eta(\cdot)$ is a non-negative function corresponding to the modulation scheme.
%\begin{theorem}
%\label{thm:Cg_GGC}
%If the instantaneous channel power $X$ of a fading channel is a GGC, then the {\codinggain} of a modulation scheme with {\cm} SER is given by
%\begin{align}
%\label{eqn:codinggain_ggc}
%\cg{X} = \left[2^{-1} \exp\left( \int\limits_{0}^{\infty}(\log u) \mu( \D u) \right) \int\limits_{0}^{\infty}  s^{-\DivOrd{X}} \eta(s) \D s \right]^{-1/\DivOrd{X}} \;,
%\end{align}
%where $\mu(\cdot)$ is the Thorin measure of the GGC, and $\eta(\cdot)$ is a non-negative function determined by the modulation scheme \cite{paper:adithyaSER}. Equivalently, the {\codinggain} is given by
%\begin{align}
%\label{eqn:codinggain_ggc_alt}
%\cg{X} = \left[2^{-1}\Gamma\left(\DivOrd{X} \right)h(0+) \int\limits_{0}^{\infty} s^{-\DivOrd{X}}\eta(s) \D s  \right]^{-1/\DivOrd{X}}\;,
%\end{align}
%where $h(\cdot)$ is obtained by representing the PDF of $X$ in the form \eqref{eqn:GGCPDF_canonical}.
%\end{theorem}
%\begin{IEEEproof}
%Using the fact that the SER is {\cm}, the average SER can be written in the form
%\begin{align}
%\AvgPe{X}{\rho} = \int\limits_{0}^{\infty} \MGF{X}{\rho s} \eta(s) \D s\; 
%\end{align} 
%where $\eta(\cdot)$ is the Levy measure of the instantaneous SER. Since $X$ is a GGC, we can substitute $\MGF{X}{\cdot}$ from \eqref{eqn:MGF_GGC_gen} to get
%\begin{align}
%\label{eqn:cgproof1}
%\cg{X} = \left[ 2^{-1}  \lim\limits_{\rho \rightarrow \infty} \rho^{\DivOrd{X}} \int\limits_{0}^{\infty}\exp\left( -\int\limits_{0}^{\infty} \log (1+ \rho s/u) \mu(\D u) \right) \eta(s) \D s \right]^{-1/\DivOrd{X}}\;,
%\end{align}
%where we have used the definition $\cg{X} := (2^{-1}\lim_{\rho \rightarrow \infty} \rho^{\DivOrd{X}} \AvgPe{}{\rho})^{-1/\DivOrd{X}}$. Assuming that the {\codinggain} is finite, it can be shown that the integrand in \eqref{eqn:cgproof1} satisfies the dominant convergence criterion, as a result of which we can commute the limit and integral to obtain
%\begin{align}
%\label{eqn:cgproof2}
%\cg{X} = \left[ 2^{-1} \int\limits_{0}^{\infty} \exp \left( \int\limits_{0}^{\infty}\log(u/s) \mu(\D u) \right) \eta(s) \D s \right]^{-1/\DivOrd{X}} \;.
%\end{align}
%The Theorem then follows, as \eqref{eqn:codinggain_ggc} is obtained from \eqref{eqn:cgproof2} using Theorem \ref{thm:DivOrdGGC}, and \eqref{eqn:codinggain_ggc_alt} can be established by using \eqref{eqn:hofzero} in \eqref{eqn:codinggain_ggc}.
%\end{IEEEproof}
%The reason behind providing two equivalent expressions for the {\codinggain} in Theorem \ref{thm:Cg_GGC} is that \eqref{eqn:codinggain_ggc_alt} is suitable for GGCs for which the PDF is available in closed form. On the other hand, there are several GGCs for which the PDF is not known in closed form, and only the Laplace transform is known. In such cases, \eqref{eqn:codinggain_ggc} can be used to obtain the {\codinggain}. Thus, we have the asymptotic average SER of any modulation scheme with a {\cm} SER for any non-degenerate GGC with finite Thorin mass given by
%\begin{align}
%\label{eqn:asymptoticSERFinal}
%\AvgPe{}{\rho} = (\cg{}\rho)^{-\DivOrd{}} + O(\rho^{-\DivOrd{}})\;.
%\end{align}
%Equation \eqref{eqn:asymptoticSERFinal} applies to modulation formats such as DPSK and $M$-PSK, when we use the corresponding $\eta(\cdot)$ function in $\cg{}$. For example, in the case of DPSK, $\eta(u) = \delta(u-1)$; for $M$-PSK, $\eta(u) = (\sin (\pi/M)/(2 \pi))I[u \geq 1]/(u\sqrt{u-\sin^{2}(\pi/M)})$ \cite {paper:adithyaSER}. As an illustration, we consider an arbitrary GGC, and derive the high SNR performance of binary-PSK (BPSK), for which $\eta(u) = (1/(2 \pi))I[u \geq 1]/(u \sqrt{u-1})$.
%\begin{example}
%\label{corr:BPSK_highSNRSER}
%The asymptotic average SER of BPSK over GGC fading channel with diversity order $\DivOrd{X} < \infty$ is given by $\AvgPe{X}{\rho} = (4 \sqrt{\pi})^{-1} h(0+)(\Gamma(\DivOrd{X}+0.5)/\Gamma(\DivOrd{X}+1))\rho^{-\DivOrd{X}}+ O(\rho^{-\DivOrd{X}-1})$, as $\rho \rightarrow \infty$.
%\end{example}
%
%Through Theorems \ref {thm:DivOrdGGC} and \ref{thm:Cg_GGC}, it is apparent that the asymptotic SER can be completely characterized in using the Thorin measure, which serves as a justification for our effort towards using $\GGC$ as a unifying model for fading distributions.
% for a fading channel where the instantaneous signal to interference power is a ratio of two Gamma RVs, which is a special case of \eqref{eqn:ParetoPDF} with $r=1$. In this case, the Thorin mass is $k_{1}$, and therefore from Theorem \ref{thm:DivOrdGGC}, the diversity order is $k_{1}$. To obtain the {\codinggain}, we substitute $\eta(u) = \delta(u-1)$ in \eqref{eqn:codinggain_ggc} to get $\cg{X} = \left( 2 \Gamma(k_{1})B(k_{2},k_{1})^{-1}\right)^{1/k_{1}}$. Consequently, the SER is given by $\AvgPe{}{\rho}=  2 \Gamma(k_{1})B(k_{2},k_{1})^{-1} \rho^{-k_{1}}, \rho \rightarrow \infty$.

%Another application of Theorem \ref{thm:Cg_GGC} is to study the monotonicity of the {\codinggain}s of GGC fading distribution families. For example, consider a Nakagami-$m$ fading channel employing DPSK. In this case, from Theorem \ref{thm:DivOrdGGC}, we find that $\DivOrd{X} = m$, and from Theorem \ref{thm:Cg_GGC} we see that the {\codinggain} is $\cg{}=2^{1/m}/m$. In other words, while the diversity order monotonically increases with $m$ in a Nakagami-$m$ channel, the {\codinggain} in fact monotonically decreases with $m$. This counter-intuitive result regarding the monotonicity of the {\codinggain} is not limited to DPSK modulation or the Nakagami-$m$ channel alone. In fact, the ordering of {\codinggain} for DPSK has an implication on the ordering of {\codinggain} for other modulation schemes as described below.
%\begin{theorem}
%\label{thm:cg_DPSK_and_Cgothers}
%Consider two GGC fading channels $X$, $Y$, for which the {\codinggain}s under DPSK are represented by $\cg{X,\mathrm{DPSK}}$ and $\cg{Y,\mathrm{DPSK}}$. Then
%\begin{align}
%\cg{X,\mathrm{DPSK}} \leq \cg{Y,\mathrm{DPSK}} \implies \cg{X,\mathrm{Q}} \leq \cg{Y,\mathrm{Q}} \;,
%\end{align}
%where $\cg{X,\mathrm{Q}}$ is the {\codinggain} of a constellation $\mathrm{Q}$ with {\cm} SER.
%\end{theorem}
%Recalling that {\cm} SERs are by definition exponentially bounded, the diversity order of a given GGC using DPSK equals that when the constellation Q is used. Therefore, assuming that the diversity order of $X$ is greater than that of $Y$ over DPSK, the same ordering follows for the constellation Q. On the other hand, if the {\codinggain}s under DPSK follow the opposite order, from Theorem \ref{thm:cg_DPSK_and_Cgothers} such an order is preserved when the modulation Q is used. Therefore, to find examples of fading distribution pairs for which the diversity order and {\codinggain} follow opposite orders under any constellation with {\cm} SER, it suffices to verify if they posses such a property under DPSK alone. Next, we discuss examples of such pairs of fading distributions.
%%In what follows, we derive a sufficient condition for the ordering of {\codinggain} of two GGC fading channels based on the increasing concave ordering.
%%\begin{theorem}
%%\label{thm:cg_decrease_DivInc}
%%Let the normalized Thorin measures of two GGCs with identical average power and identical diversity orders be $\hat{\mu}_{1}$ and $\hat{\mu}_{2}$. Consider RVs $M_{j} \sim \hat{\mu}_{j}$, $j=1,2$. If $M_{1} \orderl{icv} M_{2}$, then $\cg{1} \leq \cg{2}$.
%%\end{theorem}
%%\begin{IEEEproof}
%%To complete
%%\end{IEEEproof}
\subsection{Outage Probability}
The outage probability of a fading channel is defined as the probability that the instantaneous channel power falls below a certain threshold. This is equal to the CDF of the instantaneous channel power, and therefore for GGC fading channels where the CDF is available in closed form, the outage probability is immediate. On the other hand, when the CDF of the GGC is not available in closed form, we can still conclude that the outage probability is a logconcave function, since the CDF of a GGC is a logconcave function \cite[p. 67]{book:bondessonGGC}. In what follows, we provide an asymptotic expression for the outage probability, which shows that Thorin measure of the GGC relates to the outage probability.
\begin{proposition}
\label{thm:GGCOutageAsmyp}
Consider a GGC channel with Thorin mass $\alpha$. Then the asymptotic outage probability $P_{\mathrm{out}}(\cdot)$ is given by
\begin{align}
P_{\mathrm{out}}(x) \sim x^{\alpha}h(x)/\alpha,  
\end{align}
as $x \rightarrow 0$, where $h(\cdot)$ is as defined in \eqref{eqn:GGCPDF_canonical} or \eqref{eqn:GGCGammahxandA}.
\end{proposition}
Proposition \ref{thm:GGCOutageAsmyp} shows that the asymptotic outage probability is determined by the Thorin mass and the $h$ function.
\section{Stochastic Ordering of GGC Distributions}
\label{sec:OrderingGGCs}
\subsection{Laplace Transform Ordering of GGC}
So far, we have presented some techniques to analyze the high SNR performance of GGC fading channels. In this Section, we turn our attention to the stochastic ordering of GGC fading channels. This will help us to compare two GGC fading channels based on general performance metrics which are either completely monotone (such as SERs), or possess a completely monotone derivative (such as the ergodic capacity). Toward this end, the Laplace transform ordering framework proposed in \cite{paper:adithyaSTpaper} is employed. LT ordering between a pair of instantaneous {\effch} distributions implies that the average SER of a constellation with {\cm} SER, such as the case with MPSK and MQAM, will be ordered at all values of average SNR. In this Section, we focus on LT ordering of a pair of GGCs. 
%Within the GGC class, it is possible for us to show that LT ordering between a pair of RVs occurs if and only if the pair of RVs is ergodic capacity ordered. This is an important conclusion, because according to Lemma \ref{lem:GGCLTimpCap}, such an implication is not true in general for arbitrary nonnegative RVs. 

In the context of LT ordering of GGCs, we notice a duality between the Shannon transform ordering of the Thorin measures with the LT ordering of the fading distributions:
\begin{proposition}
\label{thm:Lt_Shannon_duality}
Let $X$ and $Y$ be two GGCs with Thorin measures $\mu_{X}$ and $\mu_{Y}$. We have $X \orderl{Lt} Y \iff \mu_{X} \orderl{gS} \mu_{Y}$.
\end{proposition}
\begin{proof}
The proof of this proposition follows from \eqref{eqn:LT_expectations} applied to GGCs.
\end{proof}

%\begin{proposition}
%\label{thm:Lt_Shannon_duality2}
%Let $X$ and $Y$ be two GGCs with Thorin measures $\mu_{X}$ and $\mu_{Y}$. We have $X \orderl{c} Y \iff \mu_{X} \orderl{gLt} \mu_{Y}$.
%\end{proposition}
%\begin{proof}
%To begin with, we observe that $X \orderl{c} Y$ occurs if and only if $\D \Cerg{X}{\rho} /\D \rho \leq \D \Cerg{X}{\rho} /\D \rho$, $\forall \rho \geq 0$. This is because $\Cerg{X}{0}=\Cerg{Y}{0}=0$, and the derivative of $\Cerg{X}{\rho}$ being point-wise smaller than $\Cerg{Y}{\rho}$ at all $\rho$ implies $\Cerg{X}{\rho} \leq \Cerg{Y}{\rho}$, $\forall \rho \geq 0$. We therefore need to find the conditions under which $\D \Cerg{X}{\rho} /\D \rho \leq \D \Cerg{X}{\rho} /\D \rho$ at all $\rho$. Using the expression for $\Cerg{X}{\rho}$ from \eqref{eqn:GGC_cerg_full}, and differentiating, we get 
%\begin{align}
%\label{eqn:GGC_LTshannon2Proof1}
%\frac{\D \Cerg{X}{\rho}}{\D \rho} \leq \frac{\D \Cerg{Y}{\rho}}{\D \rho} \iff \int\limits_{0}^{\infty} \gamma_{X}^{'}(\rho u)\frac{\exp(-u)}{u} \D u \leq \int\limits_{0}^{\infty} \gamma_{Y}^{'}(\rho u)\frac{\exp(-u)}{u} \D u \;,
%\end{align}
%where $\gamma_{X}^{'}(x) := \D \gamma_{X}(x)/\D x$, and likewise for $\gamma_{Y}^{'}(\cdot)$.
%Next, we express $\gamma_{X}^{'}(\cdot)$ in terms of the Thorin measure as
%\begin{align}
%\label{eqn:GGC_LTshannon2Proof2}
%\frac{\D}{\D \rho}\gamma_{X}(\rho u) = \int\limits_{0}^{\infty} \frac{u}{s+\rho u} \mu_{X}(\D s)\;,
%\end{align} 
%and likewise for $\D \gamma_{Y}(\rho u) / \D \rho$.
%
%Substituting \eqref{eqn:GGC_LTshannon2Proof2} in \eqref{eqn:GGC_LTshannon2Proof1} and using the identity $\int_{0}^{\infty} \exp(-u)/(s+\rho u) \D u = \rho^{-1}\exp(-s/\rho)$, we get
%\begin{align}
%\label{eqn:GGC_LTshannon2Proof3}
%\frac{\D \Cerg{X}{\rho}}{\D \rho} \leq \frac{\D \Cerg{Y}{\rho}}{\D \rho} \iff \int\limits_{0}^{\infty} \exp(-s/\rho) \mu_{X}(\D s) \leq \int\limits_{0}^{\infty} \exp(-s/\rho) \mu_{Y}(\D s)
%\end{align}
%at all $\rho >0$. This is equivalent to
%\begin{align}
%\label{eqn:GGC_LTshannon2Proof3}
%\frac{\D \Cerg{X}{\rho}}{\D \rho} \leq \frac{\D \Cerg{Y}{\rho}}{\D \rho} \iff \mu_{X} \orderl{gLt} \mu_{Y}\;.
%\end{align}
%This completes the proof.
%\end{proof}
The connection between the LT order and the Shannon transform order as suggested by Proposition \ref{thm:Lt_Shannon_duality} can be exploited in obtaining new ordering relations between GGC fading distributions, by using the properties of one stochastic order to benefit the other. For instance, by observing that $g(x) = \log(1+sx)$ is a Bernstein function, we obtain the relation $\mu_{X} \orderl{gLt} \mu_{Y} \implies \mu_{X} \orderl{gS} \mu_{Y}$, for cases when the Thorin masses of $X$ and $Y$ are identical. Now, using Proposition \ref{thm:Lt_Shannon_duality}, we conclude that $\mu_{X} \orderl{gLt} \mu_{Y} \implies X \orderl{Lt} Y$, if the diversity orders of $X$ and $Y$ are equal. Therefore, the generalized LT ordering of the Thorin measures of two GGCs with equal diversity order implies that the average SER performance at all SNR for the first one is better than that of the second at all SNR. 
%Next, we establish an important equivalence between LT ordering and ergodic capacity ordering of a subset of GGCs.
%\begin{theorem}
%\label{thm:LtErgCapOrderEquiv}
%Let $X$ and $Y$ be two GGCs with finite and equal Thorin masses. Then $X \orderl{c} Y \iff X \orderl{Lt} Y$.
%\end{theorem}
%\begin{proof}
%For any two nonnegative RVs $X$ and $Y$, we have $X \orderl{Lt} Y \implies X \orderl{c} Y$ according to Lemma \ref{lem:GGCLTimpCap}. We now prove the converse, i.e., $X \orderl{c} Y \implies X \orderl{Lt} Y$ to hold for $X$ and $Y$ when they are GGCs with finite and equal Thorin masses. First, observe from Proposition \ref{thm:Lt_Shannon_duality2} that $X \orderl{c} Y \implies \mu_{X} \orderl{gLt} \mu_{Y}$. Next, according to Property \textbf{P1}, $\mu_{X} \orderl{gLt} \mu_{Y} \implies \mu_{X} \orderl{gS} \mu_{Y}$ when the Thorin masses of $X$ and $Y$ are finite and equal. To conclude the proof, recall from Proposition \ref{thm:Lt_Shannon_duality} that $\mu_{X} \orderl{gS} \mu_{Y} \implies X \orderl{Lt} Y$. We have thus showed that when the Thorin masses of $X$ and $Y$ are finite and equal, then $X \orderl{c} Y \implies X \orderl{Lt} Y$.
%\end{proof}
%Theorem \ref{thm:LtErgCapOrderEquiv} proves for the first time that if $X \orderl{c} Y$ and $X \norderl{Lt} Y$, then the Thorin masses of $X$ and $Y$ cannot be equal. Interpreting the ergodic capacity as what is achievable by coding over an i.i.d. time-extension of the channel, this has the following interesting interpretation: If the SER of DPSK over $X$ is less than that of $Y$ at high SNR in an uncoded system, then it is possible to make the SER under $Y$ less than that of $X$ at high SNR in the presence of coding, only if the diversity order of $X$ is strictly less than that of $Y$. An example in support of this observation is the case where $X$ is Pareto distributed with parameters $(k_{1}=k_{2}=1,r_{1})$, and likewise $Y$ with parameters $(k_{1}=k_{2}=1,r_{2})$, where $r_{1} \leq r_{2}$.

%Further, assuming equal diversity orders for the two channels, it is easy to see that $\mu_{X} \orderl{icv} \mu_{Y} \implies \hat{\mu}_{X} \orderl{icv} \hat{\mu}_{Y}$. Finally, if we assume that the average channel powers of the two channels are equal, we can use Theorem \ref{thm:cg_decrease_DivInc} to conclude that 


Laplace transform ordering of GGCs can also be obtained through the observation that any nondegenerate GGC with finite Thorin mass is a gamma mixture. We therefore obtain the following theorem:
\begin{theorem}
\label{thm:LT_GGC_Mixture}
Let $X = A U_{1}$ and $Y = B U_{2}$ be two GGCs, where $A$ and $B$ are nonnegative RVs, independent of $U_{j} \sim Gamma(m_{j},1)$, $j=1,2$. Then $m_{1} \leq m_{2}$ and $A \orderl{Lt} B$ implies $X \orderl{Lt} Y$.
\end{theorem}
\begin{IEEEproof}
To begin with, observe that the LT of a Gamma RV monotonically decreases with the scale parameter, when the rate is unity. Therefore, if $U_{1}$ and $U_{2}$ are Gamma RVs with shape $m_{1}$ and $m_{2}$ respectively, and unit rate, then $U_{1} \orderl{Lt} U_{2} \iff m_{1} \leq m_{2}$. Now, if we assume that $A$ and $B$ are non-negative RVs independent of $U_{1}$ and $U_{2}$, which satisfy $A \orderl{Lt} B$, then using Lemma \ref{prelims:LT_MultivariateFn} with $g(x_{1},x_{2})= x_{1}x_{2}$, which is a Bernstein function of each argument when the other argument is viewed as a constant, the Theorem follows.
\end{IEEEproof}
While Theorem \ref{thm:Lt_Shannon_duality} connects the ordering of the Thorin measures and the LT ordering of the corresponding GGCs, on the other hand Theorem \ref{thm:LT_GGC_Mixture} enables us to LT order pairs of GGC RVs for which the Thorin measure may not be available in closed form. 
%We now present an illustrative example.
%\begin{example} 
%The Pareto distribution given by \eqref{eqn:ParetoPDF} is monotonic in the LT order with respect to the parameter $k_{1}$, when $k_{2}$ and $r \in (0,1]$ are fixed. To see this, observe that a Pareto RV with parameters $(1, k_{1} ,k_{2})$ is identical to $X_{1}/X_{2}$, where $X_{1} \sim Gamma(k_{1},1)$ and $X_{2} \sim Gamma(k_{2},1)$. Consequently, from Theorem \ref{thm:LT_GGC_Mixture}, a Pareto RV with parameters $(1,k_{1},k_{2})$ is dominated (in the LT ordering sense) by one with parameters $(1,\tilde{k}_{1},k_{2})$ for $k_{1} \leq \tilde{k}_{1}$. As a result, from \eqref{ch2:eqn:LT_order_relation_2}, a Pareto RV with parameters $(r,k_{1},k_{2})$ is smaller in the LT ordering sense than one with parameters $(r,\tilde{k}_{1},k_{2})$ for $r \in (0,1]$, since the function $g(x) = x^r$ is a c.m.d function for $r \in (0,1]$.
%\end{example}
%\begin{example}
%The Generalized gamma RV with PDF given by \eqref{eqn:GenGammDist} is monotonic in the LT order with respect to the $\epsilon$ and $c_{2}$ parameters, when $r$ is fixed. To see this, recall that the generalized gamma RV is of the form $Y^{1/r}$, where $Y \sim Gamma(\epsilon/r, c_{2})$. When $r$ is fixed, 
%\end{example}
\subsection{Convex Order and Performance Benchmarks}
It is well known that the AWGN (no fading) channel is a benchmark to the performance of any fading channel, with respect to convex or concave metrics. Within the class of GGC fading distributions, the Nakagami-$m$ fading scenario serves as a performance benchmark, as seen from the following Theorem.
\begin{theorem}
\label{thm:GammaBenchmark}
Let $X$ be a GGC with Thorin mass $D$ and mean $P$. Then $P U \orderl{cx} X$, where $U \sim Gamma(D,D)$.
\end{theorem}
\begin{IEEEproof}
According to Lemma \ref{lem:GGC_gammaMixture}, $X$ can be written as $A U$, where $U$ is Gamma distributed with shape $D$ and rate $D$, and $A$ is a nonnegative RV independent of $\Gamma$. Now, let $g$ be a convex function. Then 
\begin{align}
\label{eqn:GammaBencheqn}
\E{U}{g(\E{}{A} U)} \leq \E{}{g(X)} \;,
\end{align} 
as a consequence of Jensen's inequality. 
\end{IEEEproof}
It is now possible to see from Theorem \ref{thm:GammaBenchmark} that among all GGC fading channels with a given diversity order and unit average power, the Nakagami-$m$ fading channel forms the benchmark channel with respect to concave and convex performance metrics, because the instantaneous channel power of a Nakagami-$m$ channel is Gamma distributed with shape $m$ and rate $m$. In other words, if the diversity order of a GGC is $D$, then the average SER of any $1$-dimensional or $2$-dimensional constellation is lower bounded by that of a Nakagami-$m$ channel with $m=D$, and further, the ergodic capacity is upper bounded by that of the Nakagami-$m$ channel with $m=D$.

\subsection{Error Rate Performance Gap}
\label{sec:GGCperformanceGap}
While stochastic ordering techniques are capable of yielding GGC channel comparisons based on very general performance metrics without the need for closed form expressions, an inherent limitation of this method is that it is not possible to quantify the exact performance gap of one channel with respect to the other. In this account, the structure of the LT of a GGC makes it possible to produce a closed form expression for the SNR gain of one GGC with respect to another, when comparing the SERs at high SNR. The SNR gain of one channel with respect to another is defined as the difference between the SNR (in dB) for the asymptotic SER of the two channels to be equal, and is denoted as $\snrgap{X_{1},X_{2}}$.
\begin{theorem}
\label{thm:GGC_SNRgain}
For two GGC channels $X_{1},X_{2}$ with identical diversity orders $\DivOrd{}$ employing any modulation scheme with a {\cm} SER,
\begin{align}
\label{eqn:snrGapmu}
\snrgap{X_{1},X_{2}} = \frac{10}{\DivOrd{}} \left(\log_{10}e \right) \int\limits_{0}^{\infty} (\log u)(\mu_{2}(\D u) - \mu_{1}(\D u))\;,
\end{align}
where $\mu_{j}(\cdot)$ is the Thorin measure of $X_{j}$, $j=1,2$. Equivalently, 
\begin{align}
\label{eqn:snrGaphFunction}
\snrgap{X_{1},X_{2}} = \frac{10}{\DivOrd{}} \log_{10} \frac{h_{2}(0)}{h_{1}(0)}\;,
\end{align}
where $h_{j}(\cdot)$ are obtained from the canonical GGC PDF \eqref{eqn:GGCPDF_canonical} of $X_{j}, j=1,2$.
\end{theorem}
\begin{IEEEproof}
We will prove \eqref{eqn:snrGaphFunction} first, from which \eqref{eqn:snrGapmu} is obtained using the relation \eqref{eqn:hofzero}. Let $\rho_{1}$ and $\rho_{2}$ denote the average SNRs for channels $X_{1}$ and $X_{2}$ required to obtain the same asymptotic SER. In other words, $(\cg{1}\rho_{1})^{- \DivOrd{}} =   (\cg{2}\rho_{2})^{- \DivOrd{}}$, as $\rho \rightarrow \infty$. Relation \eqref{eqn:snrGaphFunction} then follows by taking logarithms both sides, and substituting the {\codinggain} expressions from \eqref{eqn:codinggain_ggc_alt}. 
\end{IEEEproof}
In Theorem \ref{thm:GGC_SNRgain}, we only consider channels with equal diversity order, because if the two channels have unequal diversity orders, then $\snrgap{X_{1},X_{2}}$ is infinity. 
%\section{Applications}
%Next, we present some applications of the above results in evaluating the performance metrics of multiple receive antenna diversity combining systems.
%\subsection{Diversity Combining Systems}
%Consider the $L$-branch receive diversity system model
%\begin{align}
%y_{j} = \sqrt{\rho} h_{j} s +v_{j},\; j=1,\ldots,L\;,
%\end{align}
%where $y_{j}$ is the received signal at each branch, $h_{j}$ is the independent fading across branch $j$, and $v_{j}$ is the circularly symmetric complex additive white Gaussian noise. Depending on the channel information at the receiver, the combiner may perform either maximum ratio combining, equal gain combining or selection combining. The instantaneous channel powers after combining, for each of these cases is given by $X_{\mathrm{MRC}} = \sum_{i=1}^{L} X_{i}$, $X_{\mathrm{EGC}} = L^{-1}\left(\sum_{i=1}^{L} \sqrt{X_{i}}\right)^{2}$, and $X_{\mathrm{SC}} = \max_{i=1,\ldots,L} X_{i}$ respectively. For the case of MRC, it is possible for us to quantify the Thorin measure of the combined instantaneous channel power, in terms of the Thorin measures of the component branch channel powers. This permits us to obtain the expression for the SER at all SNR, as well as quantify the diversity order and {\codinggain} using Theorems \ref{thm:DivOrdGGC} and \ref{thm:Cg_GGC}.
%\begin{proposition}
%\label{prop:MRC_thorin}
%Consider an $L$-branch MRC system with independent GGC fading across each branch. If $\mu_{i}$, $i=1,\ldots,L$ is the Thorin measure of the instantaneous channel power of branch $i$, then $\mu_{\mathrm{MRC}}(u) = \sum_{i=1}^{L} \mu_{i}(u)$.
%\end{proposition} 
%\begin{IEEEproof}
%To complete.
%\end{IEEEproof}
%As an application of Proposition \ref{prop:MRC_thorin}, consider a two-branch MRC system with independent Nakagami-$m$ fading across each branch, where $m=1$ for the first branch, and $m=3$ for the second branch. Then, from Theorem \ref{thm:AvgPwr}, the average power of the combined channel is $2$ units; the diversity order is given by Theorem \ref{thm:DivOrdGGC} as $4$, and the {\codinggain} for DPSK according to Corollary 1 of Theorem \ref{thm:Cg_GGC} is given by $2^{1/4}/4$. To illustrate an application of Theorem \ref{thm:GGC_SNRgain}, consider another two $2$-branch MRC diversity combining system with independent Nakagami-$m$ fading across the branches, where $m=2$ for both the branches. From Theorem \ref{thm:DivOrdGGC}, we see that the second system has a diversity order of $4$ as well, due to which we can use Theorem \ref{thm:GGC_SNRgain} to quantify the performance gap at high SNR, which is found to be $\snrgap{\mathrm{MRC}_{1},\mathrm{MRC}_{2}} = (5/2) \log_{10} 2^4/3^3 \approx -0.5681$ dB. We corroborate this result in Section \ref{} using Monte-carlo simulations.
%
%In the case of EGC and SC, it is not possible to obtain the Thorin measure of the combined instantaneous channel power in closed form, as it is not even a GGC, in general. Nevertheless, it is possible for us to derive asymptotic SER expressions using the following result of \cite{paper:yuanTauberian}:
%\begin{lem}
%\label{lem:yuan}
%Quote Yuan's result for SC and EGC here. Involve F(z) near origin.
%\end{lem}
%%In order to use Lemma \ref{lem:yuan} to obtain the asymptotic SER expression, we need the variation of the CDF of a GGC near the origin:
%%\begin{lem}
%%\label{lem:GGC_CDF_origin}
%%If $\CDF{X}{x}$ is the CDF of a GGC with finite Thorin mass, then $\CDF{X}{x} \sim (A/\Gamma(\DivOrd{}+1))x^{\DivOrd{}}$, where $\DivOrd{} = \int_{0}^{\infty} \mu(u) \D u$, and $\mu$ is the Thorin measure of $X$.
%%\end{lem}
%%\begin{IEEEproof}
%%To complete.
%%\end{IEEEproof}
%%We are now ready to produce the asymptotic SER expression for EGC and SC:
%%\begin{theorem}
%%For an $L$-branch diversity combining system experiencing independent GGC fading across the branches, the asymptotic average SER of any constellation with exponentially bounded SER is given by
%%\begin{align}
%%\AvgPe{}{\mathrm{EGC}}{\rho} = \\
%%\AvgPe{}{\mathrm{SC}}{\rho} = \;,
%%\end{align}
%%for EGC and SC respectively.
%%\end{theorem}
%
\section{Systems Involving Multiple GGC RVs}
\label{sec:GGCPerfBoundsSys}
Many systems of practical interest involve combinations of multiple fading components. In what follows, we find the conditions under which the overall end-to-end instantaneous channel power is a GGC (with finite Thorin measure). This permits us to obtain generic bounds on system performance metrics such as the ergodic capacity and average SER, where only asymptotic results exist in the literature. The bounds obtained herein compare the performance metric of a GGC with that of a Nakagami-$m$ channel, since the SERs and ergodic capacity are computable in closed form (see eg. \cite[pp. 222-224]{simon_alouini05}). Furthermore, we rely only on the diversity order of the system, which may be obtained through asymptotic methods, such as in \cite{paper:yuanTauberian}.

\subsection{Composite Fading Systems}
Many fading models in wireless communications attempt to capture both the short term fading effect and the long term shadowing effect through a composite fading distribution. In such cases, the instantaneous {\effch} is modelled as a product of two RVs, one corresponding to the short-term effect, and the other corresponding to the long-term fading effect. In other words, the overall instantaneous {\effch} $Z$ can be written as $Z=XY$. For such systems, $Z$ is a GGC if $X$ is a GGC and $Y$ is HCM, as seen through an application of Lemma \ref{lem:props_GGC_HCM}. The Thorin mass of $Z$ is finite if the Thorin mass of either $X$ or $Y$ is finite, as seen from Lemma \ref{prop:ggcCombFiniteThorinMass}. As a result, common composite models such as the Rayleigh-lognormal model \cite{turkmani1992probability}, the Nakagami-lognormal model \cite{ho1993co} and the Gamma-shadowed generalized Nakagami fading model \cite{alouini1999unified} have GGC instantaneous {\effch}s with finite Thorin mass. 
\subsection{Diversity Combining Systems}
\label{sec:GGCpaperDivComb}
Consider a single-input multiple-output diversity combining system with $L$ receive antennas, and complete CSI at the receiver. We now show that under different assumptions on the instantaneous channel power of each branch, the end-to-end instantaneous channel power of combining schemes such as MRC, EGC and SC is a GGC. 
\subsubsection{Maximum Ratio Combining}
In the case of MRC, the instantaneous end-to-end channel power $X_{\mathrm{MRC}} = \sum_{i=1}^{L} X_{i}$ is a GGC whenever $X_{i}$ is a GGC, since a sum of GGC RVs is a GGC. It is therefore straightforward to see that the average SER of DPSK is given by one-half $\MGF{}{\rho}$ in \eqref{eqn:MGF_GGC_gen}, where the Thorin measure is the sum of Thorin measures of each component of the MRC system. The ergodic capacity and average SERs of other $2$-dimensional modulations may however not be tractable in general, for example when the branches are independent but not identically distributed GGCs. In this case, it is possible for us to obtain a performance lower bound if the diversity order is known. To this end, from Proposition \ref{prop:ggcCombFiniteThorinMass}, if every component has finite diversity order, then the diversity order of the MRC system is finite, and is given by $D = \sum_{i=1}^{N} \int \mu_{i}(\D u)$. Now, since $X_{\mathrm{MRC}}$ is a GGC with Thorin mass $D < \infty$, using Theorem \ref{thm:GammaBenchmark}, we see that the performance of the MRC system is lower bounded by that of a Nakagami-$m$ channel with $m=D$, with respect to all convex metrics such as average SERs of $2$-dimensional modulations and concave metrics such as the ergodic capacity.
\subsubsection{Equal Gain Combining}
Next, consider an EGC system, where $X_{\mathrm{EGC}} = L^{-1}\left(\sum_{i=1}^{L} \sqrt{X_{i}}\right)^{2}$. Although it is not true in general that $X_{\mathrm{EGC}}$ is a GGC whenever $X_{i}$ is a GGC or even HCM, it can be shown that when $X_{i}$ is a product of generalized Gamma distributed RVs, $X_{\mathrm{EGC}}$ is a GGC. Closed-form expressions for the average SER and ergodic capacity in this case are intractable for many distributions such as Nakagami-$m$ and Hoyt, which are special cases of generalized Gamma distributions. In order to obtain a lower bound on the performance metrics, we see from Proposition \ref{prop:ggcCombFiniteThorinMass} that $X_{\mathrm{EGC}}$ is a GGC with finite diversity order if every branch has finite diversity order. Furthermore, the diversity order $D = \sum_{i=1}^{N} \int \mu_{i}(\D u) < \infty$. We can therefore use Theorem \ref{thm:GammaBenchmark} to bound the average SER and the ergodic capacity by that of a Nakagami-$m$ channel.
\subsubsection{Selection Combining}
On the other hand, when SC is performed, $X_{\mathrm{SC}} = \max_{i=1,\ldots,L} X_{i}$. Similar to the EGC case, it is insufficient to assume $X_{i}$ to be GGC or HCM in order to get a GGC distributed $X_{\mathrm{SC}}$. However, it can be shown that when $X_{i}$ is of the form $Y/Z$, where $Y$ is a GGC, and $Z$ is an exponential RV, then $X_{\mathrm{SC}}$ is a GGC. $X_{i}$ can be written in this form in several scenarios of interest, for example, in an interference limited system with only one dominant Rayleigh faded interference source. In such cases, it is possible to show that $X_{\mathrm{SC}}$ is also a ratio of a GGC RV and an exponential RV. The diversity order of a SC system is the same as that of an MRC system, which is given by $D = \sum_{i=1}^{N} \int \mu_{i}(\D u)$. To ensure $D$ to be finite, $ \int \mu_{i}(\D u)$ must be finite for each $i=1,\ldots,L$. In other words, the Thorin mass of each branch must be finite. Since each branch instantaneous channel power is of the form $Y/Z$, using Proposition \ref{prop:ggcCombFiniteThorinMass}, we see that it is sufficient to ensure that the Thorin mass of $Y$ is finite, since $Z$ is exponentially distributed, and has Thorin mass of $1$. Consequently, we may employ Theorem \ref{thm:GammaBenchmark} to bound the performance of an EGC system using that of a Nakagami-$m$ system.
\section{Simulations}
\label{sec:simulations}
In this section we corroborate some of our theoretical results using Monte-Carlo simulations. In Figure \ref{fig:NakagamiVsPareto2antM125}, we simulate the performance of a $2$-branch MRC system where the instantaneous channel powers are Pareto distributed with parameters $(1,1,1.25)$, and compare it with that of a SISO Nakagami-$m$ channel with $m=2.5$. The average powers of both the systems have been normalized to unity. This simulation demonstrates that the average SER of the MRC system with Pareto distributed branches, which are GGC's with finite Thorin mass is lower bounded by that of a Nakagami-$m$ channel, as suggested in Section \ref{sec:GGCpaperDivComb}.
\begin{figure}[htb]
\centering
\includegraphics[scale=0.5]{Images/NakagamiVsPareto2antM125}
\caption{Average SER performance of $2$-branch MRC with Pareto($1.25$) distributed SNR compared with that of Nakagami-$m$ SISO channel with $m=2.5$}\label{fig:NakagamiVsPareto2antM125}.
\end{figure}
\section{Conclusions}
\label{sec:conclusions}

%\subsection{Fading Channels with alpha-Stable Noise}
%We now shift our attention to fading channels with non-Gaussian noise. Specifically, the channel model is the following:
%\begin{align}
%y = \sqrt{\rho X} s + \sqrt{A}G\;,
%\end{align}
%where $s$ is the transmitted symbol, $\rho$ is the average signal power, $G \sim \mathcal{N}(0,1)$ and $A$ is a positively skewed alpha-stable RV with characteristic exponent $\alpha \in (0,1)$. In this case, the instantaneous channel power is given by $X_{\alpha} = X/A$. It is easy to see from Lemma \ref{lem:props_GGC_HCM} that whenever $X$ is a GGC, $X_{\alpha}$ is also a GGC, since $A$ is a HCM RV. 
